Price of Anarchy for Greedy Auctions

We consider auctions in which greedy algorithms, paired with first-price or critical-price payment rules, are used to resolve multi-parameter combinatorial allocation problems. We study the price of anarchy for social welfare in such auctions. We show for a variety of equilibrium concepts, including Bayes-Nash equilibrium and correlated equilibrium, the resulting price of anarchy bound is close to the approximation factor of the underlying greedy algorithm.

==> GreedyCA-combining.tex <==
\section{Combining Mechanisms}
\label{sec.combine}

%\allan{Moved refinements to appendix and kept combining mechanisms here
%for the time being. Now that I look at this a little more, maybe this should
%come after section 8? The result in Theorem 6.2 
%raises the issue of defining a randomized $\sli$ as a distribution over
%$\sli$.}


%\brendan{The results in this section are very weak, and not very aesthetically pleasing.  I'm tempted to remove the section entirely, and perhaps note the ``obvious'' fact that randomization can be use to combine two mechanisms when/if we need it.  I've commented it out for now.}
%
%\comment{  %%%  BEGIN COMMENTS

A standard technique in the design of allocation rules is to consider both a greedy rule that favours allocation of small sets, and a simple rule that allocates all objects to a single bidder, and apply whichever solution obtains the better result \cite{BGN-03,BKV-05,MN-08}.  When bidders are single-minded, such a combination rule will be incentive-compatible \cite{MN-08}.  We would like to extend our results to cover rules of this form, but %a simple example shows that 
the price of anarchy for such a rule (with either the first-price or critical-price payment scheme) may be much worse than its combinatorial approximation ratio.  Consider the following example.

\begin{example}
\label{ex.combine}
Consider the combinatorial auction problem.  Suppose $\alg$ is the non-adaptive greedy algorithm with priority rule $r(i,S,v) = v$ if $|S| \leq \sqrt{m}$, and $r(i,S,v) = 0$ otherwise.  Let $\alg'$ be the non-adaptive greedy algorithm with priority rule $r(i,S,v) = v$ if $S = M$, and 
$r(i,S,v) = 0$ otherwise.  Then $\alg'$ simply allocates the set of all objects to the player that declares the highest value for it.  Let $\alg_{max}$ be the allocation rule that applies whichever of $\alg$ or $\alg'$ obtains the better result; that is, on input $\decls$, $\alg_{max}$ returns $\alg(\decls)$ if $SW(\alg(\decls),\decls) > SW(\alg'(\decls),\decls)$, otherwise returns $\alg'(\decls)$.  It is known that $\alg_{max}$ is a $O(\sqrt{m})$ approximate algorithm \cite{MN-08}.

Our instance of the CA problem is the following.  We have $n = m \geq 2$, say with $M = \{a_1, \dotsc, a_m\}$.  Choose $\eps > 0$ arbitrarily small.  For each $i$, the private type of agent $i$, $\typei$, is the pointwise maximum of two single-minded valuation functions: one for set $\{a_i\}$ at value $1$, and the other for set $M$ at value $1 + \eps$.  An optimal allocation profile for $\types$ would assign $\{a_i\}$ to each agent $i$, for a total welfare of $m$.  

We construct a declaration profile as follows.  For each $i$, $\decli$ is the single-minded valuation function for set $M$ at value $1 + \eps$.  On input $\decls$, $\alg_{max}$ will assign $M$ to some agent, for a total welfare of $1+\eps$.  Also, $\decls$ is a pure Nash equilibrium for $\calm_1(\alg_{max})$ and $\calm_{crit}(\alg_{max})$: all agents receive a utility of $0$, and there is no way for any single agent to obtain positive utility by deviating from $\decls$.  Taking $\eps \to 0$, we conclude that the price of anarchy for any of these mechanisms is $\Om(m)$, which does not match the combinatorial $O(\sqrt{m})$ approximation ratio of $\alg_{max}$.
\end{example}

In light of the above example, we consider a different way to combine two rules: we implement each rule as a separate mechanism, then randomly choose between the two mechanisms with equal probability.  For many examples of interest (eg. combinatorial auctions, see Section \ref{appendix:applications}) the resulting randomized allocation rule obtains (in expectation) the same worst-case combinatorial approximation ratio as applying the better of the two rules for each input.  Moreover, the price of anarchy results of this paper can be made to carry over to such randomized mechanisms, as we now formalize.

Let $\alg$ be any greedy allocation rule that never allocates $M$ to any agent, and let $\alg'$ be the allocation rule that allocates $M$ to the agent $i$ that maximizes $\decli(M)$.  The restriction on $\alg$ is motivated by our intuition that $\alg$ favours allocations of small sets; it is without loss of generality for many algorithms of interest (eg. combinatorial auctions, again see Section \ref{appendix:applications}).  
We write $\calm_1(\alg,\alg')$ for the mechanism that flips a fair coin, and if it lands heads it executes $\calm_1(\alg)$, otherwise executes $\calm_1(\alg')$.  For this mechanisms, we will \emph{allow input valuations to be non-monotone} with respect to set $M$; that is, we allow declarations in which $\decli(M) < \decli(S)$ for $S \subseteq M$.  %with respect to sets from the ranges of different algorithms.  
Note then that our mechanism is not technically a direct revelation mechanism, as an agent's input is not necessarily a monotone valuation function. 

\begin{thm}
\label{thm.comb}
Suppose that $\alg,\alg'$ are as described above and $SW(\alg,\decls) + SW(\alg',\decls) \geq \frac{1}{c}SW_{opt}(\decls)$ for every declaration profile $\decls$.  Then $\calm_1(\alg,\alg')$ obtains a $2(c+O(c^2/e^c))$ approximation at every mixed BNE. 
\end{thm}
\begin{proof}
Since the portions of agent declarations relevant to $\calm_1(\alg)$ and $\calm_1(\alg')$ are independent, an agent will optimize his declaration for $\calm_1(\alg,\alg')$ by optimizing for $\calm_1(\alg)$ and $\calm_1(\alg')$ separately.  Theorem \ref{thm.mixedNE} then immediately implies the desired result, as an equilibrium for $\calm_1(\alg,\alg')$ must be a combination of an equilibrium for $\calm_1(\alg)$ and an equilibrium for $\calm_1(\alg')$.  
\end{proof}

%} %%% END COMMENTS




==> GreedyCA-repeat.tex <==
\comment{
\section{Repeated Combinatorial Auctions}
\label{chpt.repeat}

In the previous chapter we analyzed the social welfare generated by a class of greedy combinatorial auction mechanisms when agents apply strategies at equilibrium.  These results implicitly assume that agents are able to find strategies at equilibrium.  However, as has been noted elsewhere \cite{BHLR-08, GMV-05}, there are a number of reasons to believe that an equilibrium assumption is often unrealistic for algorithmic mechanism design problems.  First, equilibria are computationally difficult to find in general, and may not exist without the presence of agents who randomize over strategies for no reason other than to preserve the stability of the system.  Even when equilibria exist and can be found, it is not clear that agents will always converge to an equilibrium under repeated play, or agree on which equilibrium to follow in a single-shot game.

In this chapter, we will focus our attention on alternative models of agent behaviour that weaken the equilibrium assumption, and have gained recent interest in the algorithmic game theory literature.  These solution concepts explicitly model a \emph{repeated-game} variant of combinatorial allocation problems, in which an auction problem is resolved multiple times with the same objects and bidders. Perhaps the most well-studied modern examples of repeated auctions are auctions for advertising spaces or slots \cite{EOS-05}, but this model applies also to bandwidth auctions (such as the FCC spectrum auction), airline landing rights auctions \cite{CSS-05}, etc.  In these settings a mechanism for the (one-shot) auction problem corresponds to a repeated game to be played by the agents.  Even in settings where the auction is not explicitly repeated, we can view the repeated-game setting as modelling the process by which agents may (or may not) converge to an equilibrium via iteratively updating their strategy choices.

One may view a repeated auction as an extensive-form game, in which a strategy describes how to behave in each round given the outcomes of the previous rounds. One might then be tempted to study the Nash equilibria of this repeated-auction game.  In general, however, it is a folk theorem that almost any outcome\footnote{Specifically, one can implement any convex combination of outcomes in which each agent's expected utility is no less than the utility he could guarantee for himself regardless of how the other agents behave.} can be implemented as an equilibrium of a repeated game, and these equilibria can be unintuitive and complex.  For example, one player may threaten that unless a certain outcome occurs on a given round, then he will play in such a way to lower the utilities of the other agents (possibly to his own detriment) in subsequent rounds.  Such threat strategies can cause the emergence of equilibrium outcomes that are unsupportable in the single-shot auction.  For this reason, we do not study fully rational equilibria of the repeated auction game.  Instead, we assume a form of limited rationality that attempts to capture natural bidding behaviour.  We study two such models: external regret minimization and asynchronous best-response.

In the first model, agents can play arbitrary sequences of strategies for the repeated auction, under the assumption that they obtain low regret relative to the best fixed strategy in hindsight.  More precisely, for each bidder, the difference between the average utility obtained by the bidder and the average utility that would have been obtained by the best single declaration in hindsight must tend to $0$ as the number of auction rounds increases.  These regret-minimizing bidders can be seen as agents that learn how to bid intelligently (relative to any fixed strategy benchmark) from the bidding history of past auction iterations.  Note that we require no assumptions about the synchrony or asynchrony of updates; arbitrary sets of agents can update their strategies concurrently.  The regret-minimization assumption is motivated by the existence of simple, efficient algorithms that minimize external regret for optimization problems such as repeated auctions \cite{KV-05,KKL-07}.  Under this model, our goal is to design an auction mechanism that achieves an approximation to the optimal social welfare \emph{on average} over sufficiently many rounds of the repeated auction.  This is precisely the problem of designing a mechanism with bounded \emph{price of total anarchy}, as introduced by Blum et al \cite{BHLR-08}.

In the second model, we assume that agents choose strategies that are myopic best-responses to the current strategies of the other agents.  Such bidding behaviour is best motivated in settings where agents update their declarations asynchronously (i.e.~not concurrently).  We model this behaviour as follows: on each auction round, an agent is chosen uniformly at random, and that agent is given the opportunity to change his strategy to the current myopic best-response.  As in the regret-minimization model, our goal is to design auction mechanisms that achieve approximations to the best possible social welfare \emph{on average} over sufficiently many auction rounds, with high probability over the random choices of bidders to update.  This is closely related to the concept of the \emph{price of (myopic) sinking}, as introduced by Goemans et al \cite{GMV-05}.  One method for bounding the price of sinking is to prove that there exists an equilibrium state that is reachable from any declaration profile by some polynomial-length sequence of best-response steps.  This would imply that an equilibrium state would be reached with high probability after exponentially many steps.  We do not take this approach, but rather prove the stronger result that the average social welfare obtained after a \emph{polynomial} number of steps will approximate the optimal welfare with high probability.

Our high-level goal is to decouple computational issues from incentives issues.  A full (and admittedly ambitious) solution in our domain would be a black-box conversion of a given approximation algorithm into a mechanism that implements\footnote{Throughout the paper we use the term ``implement'' in the economic sense of constructing a mechanism that obtains the desired properties when used by rational agents.} the same approximation ratio, on average over sufficiently many auction rounds, given our model of bidder behaviour.  The primary question raised in this chapter, which we partially address, is to what extent such implementations are possible.

As in sections \ref{XXX,YYY}, we design mechanisms that are based on a class of greedy approximation algorithms.  Our goal is to convert a given approximation algorithm into a mechanism without loss in performance guarantees when agents behave in accordance to our model of rationality.  What we find, loosely speaking, is that greedy approximation algorithms for combinatorial auction problems can be easily converted into mechanisms for regret-minimizing or myopic bidders.

\paragraph{Results}
Our first result is that any monotone greedy $c$-approximate algorithm can be implemented as a mechanism with price of total anarchy at most $c+1$.  
Our mechanism is a black-box reduction from an algorithm for a one-shot auction iteration, and the same mechanism is applied each auction round.  The form of our mechanism is very simple: on each round, it applies a simple modification to the bidders' declarations, then runs the approximation algorithm on the modified declarations and charges critical prices.  This mechanism is quite similar to the mechanism $\mech_{crit}(\alg)$ introduced in Chapter \ref{chpt.bne}; the purpose of our modification is to reduce the complexity of the regret minimization problem for the agents.  As in Chapter \ref{chpt.bne}, our results make use of the property of strong loser-independence, which is satisfied by greedy algorithms.

Our implementation does not depend on the specific algorithms used by the agents to minimize their regret; only that their regret vanishes as the number of rounds increases.  The rate of convergence to our approximation bound will depend on the rate at which the agents' regret vanishes.  

We also show that our mechanism is robust against various perturbations of our equilibrium concept.  First, we demonstrate that our mechanism is resilient to the presence of irrational agents, in the following sense.  If each agent either applies regret-minimizing strategies or makes arbitrary declarations (but never declares more than his true value for a set), then the mechanism attains a $c+1$ approximation to the optimal welfare \emph{obtainable by the regret-minimizing bidders}.  The no-overbidding assumption is necessary (as otherwise a irrational agent could bid arbitrarily highly and prevent any welfare from being obtained) and motivated by viewing irrational players as not understanding how to participate intelligently in the auction and thus likely to bid conservatively.

We also show that our performance bound degrades gracefully if agents can only approximately minimize their regret.  For $\gamma \geq 1$, if each agent is assumed to obtain a $\gamma$-approximation to the average utility of the single best strategy in hindsight, then our mechanism will obtain a $c+\gamma$ approximation to the optimal welfare (in addition to the additive error due to regret that vanishes as the number of rounds grows).  

We then consider the best-response model, in which we focus specifically on the general combinatorial auction problem.  
We present a mechanism that implements an $O(s)$ approximation for cardinality-restricted combinatorial auctions where set allocations have size at most $s$, then extend this to a mechanism that implements an $O(\sqrt{m})$ approximation for general combinatorial auctions.  We attain these approximation ratios with high probability after polynomially many auction rounds (in fact, only a slightly superlinear number of rounds). 

We conjecture that the black-box reduction used to obtain a $c+1$ approximation in the regret-minimization setting also implements an $O(c)$ approximation, on average over sufficiently many rounds, in the model of best-response bidders.  We leave this conjecture as an open problem. 

Our results require a mild game-theoretic assumption, which is that bidders will not apply strategies that are (strictly) dominated by easily-found alternatives.  This is precisely the assumption of algorithmically undominated strategies, as introduced by Babaioff et al \cite{BLP-09}\footnote{As discussed in Section \ref{sec:regret}, this assumption is not without loss of generality, but is intuitively motivated by the observation that the adoption of a dominated strategy corresponds to unnaturally risky bidding behaviour with no benefit.}.  Additionally, the mechanism for best-response bidders applies a technique known in implementation theory as \emph{virtual implementation}, where an alternative social choice rule is applied with vanishingly small probability \cite{J-01}.  We view this not as an introduction of randomness into the algorithm being implemented, but rather as the introduction of a trembling-hand consideration into the solution concept that encourages reasonable behaviour when best-response agents must distinguish between otherwise equally beneficial strategies.

} %End of first comment

\comment{
\paragraph{Related Work}
Truthful mechanisms for the combinatorial auction problem have been extensively studied.  For general CAs,
%A lower bound going back to 
Hastad's well-known inapproximability result \cite{HAS-97} 
shows that it is hard to approximate the problem to within $\Om(\sqrt{m})$ assuming $NP \neq ZPP$.  
%An alternative bound by Nisan \cite{NIS-02} shows that exponential communication is necessary to approximate general CAs to within $\Om(\sqrt{m})$, independent of complexity assumptions.  
The best known deterministic truthful mechanism for CAs with general valuations 
%is a bundling auction that 
attains an approximation ratio of $O(\frac{m}{\sqrt{\log m}})$ \cite{HKNS-04}.  A randomized $O(\sqrt{m})$-approximate mechanism that is truthful in expectation was given by Lavi and Swamy \cite{LS-05}.  Dobzinski, Nisan and Schapira \cite{DNS-06} then gave an $O(\sqrt{m})$-approximate universally truthful randomized mechanism.

Many variations on the combinatorial auction problem have been considered in the literature.  Bartal et al \cite{BGN-03} give a truthful $O(m^{\frac{1}{B-2}})$ mechanism for multi-unit combinatorial auctions with $B$ copies of each object, for all $B \geq 3$.  Dobzinski and Nisan \cite{DN-07} construct a truthful $2$-approximate mechanism for multi-unit auctions, and Dobzinski et al construct a randomized PTAS for the multi-unit auction problem that is truthful in expectation. %(ie. having many copies of just a single object),
%with general valuations
%and a truthful PTAS when additionally each declaration is $k$-minded (i.e. can be represented as the maximum of $k$ single-minded desires).  
Many other problems have truthful mechansisms  
(\cite{LOS-99, MN-08, BKV-05}) 
%are known for cases 
when bidders are restricted to being single-minded.  

Implementation at equilibrium, especially for the alternative goal of profit maximization, has a rich history in the economics literature; see, for example, Jackson \cite{J-01} for a survey.
The problem of designing combinatorial auction mechanisms that implement approximations at equilibria (and, in particular, Bayes-Nash equilibria for partial information settings) was considered by Christodoulous et al \cite{CKS-08} for submodular CAs.  Lucier and Borodin \cite{BL-10} gave a black-box implementation for a class of greedy approximation algorithms for general CA problems, with very little loss to approximation ratios.  This latter paper is similar in spirit to the current work; its construction implements a $c$-approximation algorithm as a one-shot $c(1+o(1))$-approximate mechanism at equilibrium.  However, in that work, the process by which such an equilibrium is reached is left open.  The current paper can be viewed as a demonstration that a similar sort of reduction is possible in various alternative solution concepts, even when convergence to equilibrium is not guaranteed.

The study of regret-minimization goes back to the work of Hannan on repeated two-player games \cite{H-57}.  Kalai and Vempala \cite{KV-05} extend the work of Hannan to online optimization problems, and Kakade et al \cite{KKL-07} further extend to settings of approximate regret minimization.  Blum et al \cite{BHLR-08} apply regret-minimization to the study of inefficiency in repeated games, coining the phrase ``price of total anarchy'' for the worst-case ratio between the optimal objective value and the average objective value when agents minimize regret.

Properties of best-response dynamics in repeated games, and especially the question of convergence to a pure equilibrium, is well-studied (see Chapter 19 of \cite{AGT}).  The study of average performance of best-response dynamics as a metric of game inefficiency, the so-called ``price of sinking,'' was introduced by Goemans et al \cite{GMV-05}.

Babaioff et al \cite{BLP-09} study implementation of algorithms in undominated strategies, which is a relaxation of the dominant strategy truthfulness concept.  They focus on a variant of the CA problem in which agents are assumed to have ``single-value'' valuations, and present a mechanism to implement such auctions in a multi-round fashion.  By comparison, mechanisms in our proposed model solve each instance of an auction in a one-shot manner, and our solution concept assumes that the auction is repeated multiple times.
}

\comment{  %% BEGIN COMMENTING PRELIMINARIES

\subsection{Preliminaries}

\subsubsection{Repeated Auctions}

We consider an instance of a combinatorial allocation problem that proceeds in rounds.  The problem will be resolved by a direct revelation mechanism $\mech$, say with allocation algorithm $\alg$, which independently executes on each round of the auction.  As usual, we will tend to write $\allocs$ for the allocation rule associated with algorithm $\alg$.  We will make use of the definitions of \emph{greedy} algorithms and \emph{strongly loser-independent} algorithms from 
section \ref{sec:prelim}.

We assume that neither the agent types nor the mechanism changes between rounds of the auction.  When the agents have types $\types$ and $D = (\decls^1, \decls^2, \dotsc, \decls^T, \ldots)$ is a sequence of declared valuation profiles, we will write $SW_{\alg}(D) = \frac{1}{T}\sum_t SW(\allocs(\decls^t),\types)$ for the average welfare obtained over all declarations in $D$.  We will sometimes replace subscript $\alg$ by $\mech$, in which case the social welfare is for the allocation rule of $\mech$.

Declaration sequence $D = (\decls^0, \decls^1, \dotsc, \decls^T)$ \emph{minimizes external regret} for agent $i$ if, for any fixed declaration $\decli$, $\sum_t \utili(\decl_i^t,\declsmi^t) \geq \sum_t \utili(\decli,\declsmi^t) + o(T)$.  That is, the utility of agent $i$ approaches the utility of the optimal fixed strategy in hindsight.

Declaration sequence $D = (\decls^0, \decls^1, \dotsc, \decls^T)$ is an instance of \emph{response dynamics} if, for all $1 \leq t \leq T$, profiles $\decls^{t-1}$ and $\decls^t$ differ on the declaration of at most one player.  Response dynamics $D$ is an instance of \emph{best-response dynamics} if, whenever $\decls^{t-1}$ and $\decls^t$ differ on the declaration of agent $i$, $\decl_i^t$ maximizes agent $i$'s utility given the declarations of the other bidders. That is, $\decl_i^t \in \argmax_{\decl}\{\utili(\decl,\declsmi^t)\}$.

\subsubsection{Regret Minimization} 

We now describe the concept of external regret minimization in further detail.  The external regret of a sequence of declarations is the difference between the average utility of an agent (i.e.~value of goods received minus payment extracted) and the maximum average utility that could have been obtained by a single fixed declaration made each round.  An algorithm for generating declarations is regret-minimizing if its regret vanishes as a function of the number of auction rounds.

Our bounds on mechanism performance depend upon the agents actually minimizing their external regret, but how reasonable is it to assume that agents will do so?  We recall that there is a simple and efficient algorithm for minimizing regret due to Kalai and Vempala \cite{KV-05} for minimizing regret, known as ``follow the perturbed leader,'' which runs in time polynomial in the number of actions that can be taken by the agent.  They also provide an improved algorithm that minimizes regret for a linear optimization problem, which runs in time polynomial in the problem dimension.  These algorithms require access to an exact best-response oracle, which chooses the strategy that maximizes utility given the expected outcomes of each strategy.  Kakade et al \cite{KKL-07} show how to use a $\gamma$-approximate best response oracle to achieve a $\gamma$-approximation to the best fixed declaration in hindsight.  

The regret-minimization mechanism we construct in this paper will reduce the
strategy space for a bidder to an optimization problem over the space of possible allocations to that bidder.  Using a follow-the-perturbed-leader approach, an agent can therefore minimize regret in time proportional to the number of desired sets in his valuation function.  If we assume the number of desired sets for each agent is polynomially small (e.g. in the model where agents provide these bids explicitly to the auction algorithm), then we conclude that agents can minimize regret efficiently.
Alternatively, one could provide access to a best-response (or approximate best-response) oracle for the approximation algorithms being implemented, where the oracle must compute a best response to a distribution over possible declarations of the other agents.
The ability to compute best-response choices is also a necessary component for the setting of best-response bidders, where the best-response assumption certainly requires that such strategies can be found efficiently.  

In general, however, the space of possible allocations is exponentially large, and has exponential dimension as a linear problem.  Thus, any efficient best-response oracle (to a distribution over possible declarations of the other bidders) must depend on the model by which agents access their own preferences and the details of the problem setting and algorithm being implemented.  We leave the construction of such oracles to the designers of mechanisms for specific problem domains.

\subsubsection{Related Work}

Truthful mechanisms for the combinatorial auction problem have been extensively studied.  For general CAs,
%A lower bound going back to 
Hastad's well-known inapproximability result \cite{HAS-97} 
shows that it is hard to approximate the problem to within $\Om(\sqrt{m})$ assuming $NP \neq ZPP$.  
%An alternative bound by Nisan \cite{NIS-02} shows that exponential communication is necessary to approximate general CAs to within $\Om(\sqrt{m})$, independent of complexity assumptions.  
The best known deterministic truthful mechanism for CAs with general valuations 
%is a bundling auction that 
attains an approximation ratio of $O(\frac{m}{\sqrt{\log m}})$ \cite{HKNS-04}.  A randomized $O(\sqrt{m})$-approximate mechanism that is truthful in expectation was given by Lavi and Swamy \cite{LS-05}.  Dobzinski, Nisan and Schapira \cite{DNS-06} then gave an $O(\sqrt{m})$-approximate universally truthful randomized mechanism.

Many variations on the combinatorial auction problem have been considered in the literature.  Bartal et al \cite{BGN-03} give a truthful $O(m^{\frac{1}{B-2}})$ mechanism for multi-unit combinatorial auctions with $B$ copies of each object, for all $B \geq 3$.  Dobzinski and Nisan \cite{DN-07} construct a truthful $2$-approximate mechanism for multi-unit auctions, and Dobzinski et al construct a randomized PTAS for the multi-unit auction problem that is truthful in expectation. %(ie. having many copies of just a single object),
%with general valuations
%and a truthful PTAS when additionally each declaration is $k$-minded (i.e. can be represented as the maximum of $k$ single-minded desires).  
Many other problems have truthful mechansisms  
(\cite{LOS-99, MN-08, BKV-05}) 
%are known for cases 
when bidders are restricted to being single-minded.  Borodin and Lucier \cite{BL-10} study the limited power of certain classes of greedy algorithms for truthfully approximating CA problems.

Implementation at equilibrium, especially for the alternative goal of profit maximization, has a rich history in the economics literature; see, for example, Jackson \cite{J-01} for a survey.
The problem of designing combinatorial auction mechanisms that implement approximations at equilibria (and, in particular, Bayes-Nash equilibria for partial information settings) was considered by Christodoulous et al \cite{CKS-08} for submodular CAs.  Lucier and Borodin \cite{BL-10b} gave a black-box implementation for a class of greedy approximation algorithms for general CA problems, with very little loss to approximation ratios.  This latter paper is similar in spirit to the current work; its construction implements a $c$-approximation algorithm as a one-shot $c(1+o(1))$-approximate mechanism at equilibrium.  However, in that work, the process by which such an equilibrium is reached is left open.  The current paper can be viewed as a demonstration that a similar sort of reduction is possible in various alternative solution concepts, even when convergence to equilibrium is not guaranteed.

The study of regret-minimization goes back to the work of Hannan on repeated two-player games \cite{H-57}.  Kalai and Vempala \cite{KV-05} extend the work of Hannan to online optimization problems, and Kakade et al \cite{KKL-07} further extend to settings of approximate regret minimization.  Blum et al \cite{BHLR-08} apply regret-minimization to the study of inefficiency in repeated games, coining the phrase ``price of total anarchy'' for the worst-case ratio between the optimal objective value and the average objective value when agents minimize regret.

Properties of best-response dynamics in repeated games, and especially the question of convergence to a pure equilibrium, is well-studied (see Chapter 19 of \cite{AGT}).  The study of average performance of best-response dynamics as a metric of game inefficiency, the so-called ``price of sinking,'' was introduced by Goemans et al \cite{GMV-05}.

Babaioff et al \cite{BLP-09} study implementation of algorithms in undominated strategies, which is a relaxation of the dominant strategy truthfulness concept.  They focus on a variant of the CA problem in which agents are assumed to have ``single-value'' valuations, and present a mechanism to implement such auctions in a multi-round fashion.  By comparison, mechanisms in our proposed model solve each instance of an auction in a one-shot manner, and our solution concept assumes that the auction is repeated multiple times.

%\section{Model and Definitions}

\subsubsection{Feasible Allocation Problems}

In general we will use boldface to represent vectors, subscript $i$ to denote the $i$th component, and subscript $-i$ to denote all components except $i$, so that, for example, $\vals = (\vali,\valsmi)$.  %A \emph{combinatorial allocation 

We consider the domain of combinatorial auction problems, where $n$ agents desire subsets of a set $M$ of $m$ objects.  An \emph{allocation profile} is a collection of subsets $X_1, \dotsc, X_n$, where $X_i$ is thought of as the subset allocated to agent $i$.  A particular problem instance is defined by the set of \emph{feasible allocation profiles} that are permitted. For example, the general combinatorial auction problem requires that all allocated subsets be disjoint.  Each agent $i$ has a privately-held \emph{valuation function} $\typei : 2^M \to \reals$, his \emph{type}, that assigns a value to each allocation.  We assume that valuation functions are monotone and normalized so that $\val(\emptyset) = 0$.  
A valuation function $\val$ is \emph{single-minded} if there exists $S \subseteq M$ and $x \geq 0$ such that $\val(T) = x$ if $S \subseteq T$ and $\val(T) = 0$ otherwise.  We will write $\emptyset$ for the zero valuation, and $(S,x)$ for a single-minded declaration for $S$ at value $x$.

An \emph{allocation rule} $\alg$ assigns to each valuation profile $\vals$ a feasible outcome $\alg(\vals)$; we write $\alg_i(\vals)$ 
for the allocation to agent $i$.  
We write $\alg$ for both an allocation rule and an algorithm that implements it.

An allocation rule is \emph{loser-independent} if, whenever $\valsmi$, $\valsmi'$ satisfy $\alg(\emptyset,\valsmi) = \alg(\emptyset,\valsmi')$ and  $\val_j(\alg_j(\emptyset,\valsmi)) = \val_j(\alg_j(\emptyset,\valsmi'))$ for all $j \neq i$, then $\alg(\vali,\valsmi) = \alg(\vali,\valsmi')$.  In other words, agent $i$'s perception of the behaviour of $\alg$ depends only on those agents who would win if agent $i$ did not participate, and on their declared values for their winnings.

A payment rule $P$ assigns a vector of $n$ payments to each valuation profile.  A \emph{direct revelation mechanism} $\mech$ is composed of an allocation rule $\alg$ and a payment rule $P$.  The mechanism proceeds by eliciting a valuation profile $\decls$ of \emph{declarations} from the agents, then applying the allocation and payment rules to $\decls$.  
The utility of agent $i$ for mechanism $\calm$, given declaration profile $\decls$, is $\utili(\decls) = \typei(\alg_i(\decls)) - P_i(\decls)$.  We think of each agent as wanting to choose $\decli$ to maximize $\utili(\decls)$.

The \emph{social welfare} obtained by allocation profile $\ballocs$, given type profile $\types$, is $SW(\ballocs,\types) = \sum_i \typei(\balloci)$. Given fixed type profile $\types$, we write $SW_{opt}$ for $\max_{\ballocs}\{SW(\ballocs,\types)\}$, and $SW_\alg(\decls) = \sum_i \typei(\alg(\decls))$.  When $D = (\decls^1, \decls^2, \dotsc, \decls^T)$ is a sequence of valuation profiles, we write $SW_\alg(D) = \frac{1}{T}\sum_t SW_\alg(\decls^t)$ for the average welfare obtained over all declarations in $D$.  We will sometimes replace subscript $\alg$ by $\mech$, in which case the social welfare is for the allocation rule of $\mech$.  Note that algorithm $\alg$ is a $c$-approximation if $SW_\alg(\types) \geq \frac{1}{c}SW_{opt}$ for all $\types$.  

}

\comment{

Given allocation rule $\alg$, agent $i$, declaration profile $\declsmi$, and set $S$, the \emph{critical price} $\criti^\alg(S,\declsmi)$ for $S$ is the minimum value that agent $i$ could bid on set $S$ and be allocated $S$ by $\alg$ given fixed $\declsmi$.  That is, $\criti(S,\declsmi) = \inf\{ v : \exists \decli, \decli(S) = v, \alg_i(\decli, \declsmi) = S\}.$

We say that a declaration $\decli$ is \emph{weakly dominated} by declaration $\decli'$ for agent $i$ if $\utili(\decli,\declsmi) \leq \utili(\decli',\declsmi)$ for all $\declsmi$, and furthermore there exists some $\decls_{-i}'$ such that $\utili(\decli,\decls_{-i}') < \utili(\decli',\decls_{-i}')$.  

}

%%%  END REMOVED PRELIMINARIES %%%

%\section{Repeated CAs and Regret-Minimizing Bidders}
%\label{sec:regret}
%
%\brendan{Overall we need to spend some time integrating the regret-minimizing section with the BNE section.  The arguments and concepts are all very similar; there should be significantly more sharing of lemmas, etc.}
%
%In this section we prove that if agents avoid algorithmically dominated strategies and minimize external regret, then a strongly loser-independent monotone algorithm $\alg$ can be converted into a mechanism with almost no loss to its average approximation ratio over many rounds.  The mechanism, $\mech_{crit}^{*}(\alg)$, is described in Figure \ref{fig.mech.regret}.
%Mechanism $\mech_{crit}^{*}(\alg)$ proceeds by first simplifying the declaration given by each agent, then passing the simplified declarations to algorithm $\alg$.  The resulting allocation is paired with a payment scheme that charges critical prices.  
%%
%
%\begin{figure}
%\begin{center}
%	\fbox{
%		\begin{minipage}{0.95\linewidth}
%
%\textbf{Mechanism} $\mech_{crit}^{*}(\alg)$:
%\medskip
%\hrule
%
%\medskip
%
%\textbf{Input:} Declaration profile $\decls = \decl_1, \dotsc, \decl_n$.
%
%%\textbf{Output:} A partition $X_1, \dotsc, X_n$ of $M$.
%%
%\begin{tabbing}
%1. \= $\decl' \leftarrow $ \texttt{SIMPLIFY}$(\decls)$. \\
%2. \> Allocate $\alg(\decls')$, charge critical prices.% and charge prices $p_1, \dotsc, p_n$.
%\end{tabbing}
%		\end{minipage}
%	}
%	\fbox{
%		\begin{minipage}{0.95\linewidth}
%
%\textbf{Procedure} \texttt{SIMPLIFY:}
%\medskip
%\hrule
%
%\medskip
%\textbf{Input:} Declaration profile $\decls = \decl_1, \dotsc, \decl_n$.
%
%%\textbf{Output:} A partition $X_1, \dotsc, X_n$ of $M$.
%%
%\begin{tabbing}
%1. \= For each $i \in [n]$: \\
%2. \> \quad \= Choose $S_i \in \argmax_S\{\decli(S)\}$, breaking \\ 
%\>\> ties in favour of smaller sets. \\
%3. \> \> $\decli' \leftarrow (S_i,\decli(S_i))$. \\
%4. \> Return $(\decl_1', \dotsc, \decl_n')$.
%\end{tabbing}
%		\end{minipage}
%	}
%
%			\caption[A mechanism for regret-minimizing bidders]{A mechanism for regret-minimizing bidders, based on monotone algorithm $\alg$.}
%			\label{fig.mech.regret}
%	\end{center}
%\end{figure}
%
%The simplification process \texttt{SIMPLIFY} essentially converts any declaration into a single-minded declaration (and does not affect declarations that are already single-minded).  We can therefore assume without loss of generality that agents always make single-minded declarations to this mechanism, as additional information is not used.\footnote{We note, however, that this is not the same as assuming that agents are single-minded; our results hold for bidders with general private valuations.} 
%
%Fix a particular combinatorial auction problem and type profile $\types$, and let $\alg$ be some monotone approximation algorithm.  Since $\vals$ is fixed, we can think of a strategy for each agent $i$ as a declaration $\decli \in V_i$.  Let $\decls$ be a declaration profile; we suppose each $\decli$ is a single-minded bid for set $S_i$ (and, in general, we will write $S_i$ for the set declared for in declaration $\decli$).
%We draw the following conclusion about the bidding choices of rational agents.
%
%\begin{lem}
%\label{lem.undom1}
%Let $\alg$ be a monotone approximation algorithm, and fix type profile $\types$.
%Then for each agent $i$, a single-minded declaration $\decli$ for set $S_i$ is an undominated strategy for mechanism $\mech_{crit}^{*}(\alg)$ if and only if $\decli(S_i) = \typei(S_i)$.
%\end{lem}
%\begin{proof}
%Fix some $\declsmi$ and suppose $\decli$ is a single-minded declaration for set $S_i$ 
%On input $(\decli,\declsmi)$, mechanism $\mech_{crit}^{*}(\alg)$ either allocates $S_i$ or $\emptyset$ to agent $i$.  
%Thus agent $i$'s utility for declaring $\decli$, $\utili(\decli,\declsmi)$, is $\typei(S_i) - \crit_i(S_i,\declsmi)$ when $\decli(S_i) > \crit_i(S_i,\declsmi)$, and $0$ otherwise (where $\criti$ denotes critical prices with respect to $\mech_{crit}^{*}(\alg)$).  A declaration of $\decli(S_i) = \typei(S)$ therefore maximizes $\utili(\decli,\declsmi)$ for all $\declsmi$.
%
%Next suppose that $\decli(S_i) \neq \typei(S_i)$; we will show that $\decli$ is not undominated.  Let $\decli'$ be the single-minded declaration for $S_i$ at value $\typei(S_i)$.  Suppose there is some $\declsmi$ such that $\criti^\alg(S_i,\declsmi)$ lies strictly between $\decli(S_i)$ and $\typei(S_i)$.  For simplicity we will assume such a $\declsmi$ exists; handling the general case requires only a technical extension of notation\footnote{If $\criti^\alg(S_i,\declsmi)$ never lies between $\decli(S_i)$ and $\typei(S_i))$ for any $\declsmi$, then $\mech_\alg(\decli,\declsmi) = \mech_\alg(\decli',\declsmi)$ for all $\declsmi$, so $\decli$ and $\decli'$ are equivalent strategies.  We can therefore think of $\decli$ as being ``the same'' as a single-minded declaration for $S_i$ at value $\typei(S_i)$.  We will ignore this technical issue for the remainder of the thesis, in the interest of clarity.}.  Then if $\decli(S_i) < \typei(S_i)$, then $\utili(\decli',\declsmi) > 0 = \utili(\decli,\declsmi)$.  Otherwise, if $\decli(S_i) > \typei(S_i)$), then $\utili(\decli',\declsmi) \geq 0 > \utili(\decli,\declsmi)$.  Thus, in either case, we have $\utili(\decli',\declsmi) > \utili(\decli,\declsmi)$, and therefore
%declaration $\decli'$ strictly dominates declaration $\decli$.  
%\end{proof}
%
%One implication of Lemma \ref{lem.undom1} is that the strategic choice of an agent participating in mechanism $\calm_\alg$ reduces to choosing a single set upon which to bid.  On each round, we can think of agent $i$ as choosing set $S_i$, which is the set he will attempt to win that round.  Once $S_i$ is chosen, an undominated declaration for agent $i$ is determined: the single-minded declaration for $S_i$ at value $\typei(S_i)$.  Given that agent $i$ chooses set $S_i$, his utility will be $\typei(S_i)-w_i$, where $w_i = \min\{\typei(S_i),\crit_i^\alg(S_i,\declsmi)\}$ is the price for set $S_i$, determined by the declarations of the other agents, capped at $\typei(S_i)$.  
%%Thus, since utilities are linear in the choice of $S_i$, agents can indeed apply the regret-minimization algorithm of Kalai and Vempala \cite{KV-05} to choose strategies that minimize external regret.  
%Agents can then indeed apply the regret-minimization algorithm of Kalai and Vempala \cite{KV-05} to choose strategies that minimize external regret: they need simply maintain the expected payoff for the strategy of bidding upon each of their desired sets.
%The runtime of this algorithm is polynomial in the number of sets that agent $i$ might bid upon; that is, if agent $i$ has a type with $k$ desired sets, then he can minimize his expected regret in time polynomial in $k$ (i.e.\ the number of bids required to represent his valuation in the XOR bidding language).
%
%We now proceed with bounding the social welfare obtained by $\calm_\alg$.  Let $\mathbf{y}$ be an optimal assignment for types $\types$.  Suppose that $D = \decls^1, \dotsc, \decls^T$ is a sequence of declarations to our mechanism.  The definition of regret minimization then immediately implies the following. 
%
%\begin{lem}
%\label{lem.minregret}
%If agent $i$ minimizes his external regret in bid sequence $D$, then 
%\[\frac{1}{T}\sum_t (\typei(\alg(\decls^t)) + \criti^\alg(y_i,\declsmi^t)) \geq \typei(y_i) - o(1).\]
%\end{lem}
%\begin{proof}
%Let $\decl'$ be the single-minded declaration for set $y_i$ at value $\typei(y_i)$.  From the definition of regret minimization,
%\begin{align*}
%\frac{1}{T}\sum_t & \utili(\decli^t,\declsmi^t) \geq \frac{1}{T}\sum_t \utili(\decl',\declsmi^t) - o(1) \\
%& \geq \frac{1}{T}\sum_t \left(\typei(y_i) - \criti^\alg(y_i,\declsmi^t)\right) - o(1) \\
%& = \typei(y_i) - \frac{1}{T}\sum_t \criti^\alg(y_i,\declsmi^t) - o(1).
%\end{align*}
%Since $\utili(\decli^t,\declsmi^t) \leq \typei(\alg(\decls^t))$ for all $t$, the result follows.
%\end{proof}
%
%Assume now that algorithm $\alg$ is strongly loser-independent.  We now recall from Lemma \ref{lem.greedy} that we can relate the value of the solution returned by an algorithm to the critical prices of the sets in an optimal solution.  For completeness we restate this as Lemma \ref{lem.loserindep}.
%
%\begin{lem}
%\label{lem.loserindep}
%If $\alg$ is a $c$-approximate strongly loser-independent algorithm, then for any type profile $\vals$ and optimal allocation profile $\mathbf{y}$, $\sum_{i \in [n]}\vali(\alg_i(\vals)) \geq \frac{1}{c} \sum_{i \in [n]} \criti(y_i, \valsmi)$.
%\end{lem}
%
%%\begin{lem}
%%\label{lem.loserindep}
%%For every monotone loser-independent $c$-approximate algorithm $\alg$ and allocation profile $\mathbf{y}$, \[\sum_i \decli(\alg(\decls)) \geq \frac{1}{c}\sum_i \crit_i(y_i,\declsmi).\]
%%\end{lem}
%%\begin{proof}
%%Choose some $\eps > 0$.  For each $i$, let $\decli'$ be the pointwise maximum between $\decli$ and the single-minded declaration for set $y_i$ at value $\crit_i(y_i,\declsmi) - \eps$.  The loser independence property implies that we can perform this operation independently for each agent  without affecting critical prices, and moreover $\alg(\decls') = \alg(\decls)$.  Since $\alg$ is a $c$-approximate algorithm, $\sum_i \decli'(\alg(\decls')) \geq \frac{1}{c}\sum_i \decli'(A_i) \geq \frac{1}{c}\sum_i (\crit_i(y_i,\declsmi)-\eps)$.  Additionally, since $\decli'(T) = \decli(T)$ whenever $\decli(T) \geq \crit_i(T,\declsmi)$ (from the definition of $\decli'$), we have $\decli'(\alg(\decls')) = \decli(\alg(\decls))$ for all $i$.  We conclude that $\sum_i \decli(\alg(\decls)) \geq \frac{1}{c}\sum_i (\crit_i(y_i,\declsmi)-\eps)$ for all $\eps > 0$, as required.
%%\end{proof}
%
%Furthermore, we recall from Lemma \ref{lem.greedy1} that all greedy algorithms are strongly loser-independent.  We are now ready to proceed with bounding the price of total anarchy for mechanism $\mech_{crit}^{*}(\alg)$.  
%
%\begin{thm}
%\label{thm.regretmin}
%For any monotone greedy $c$-approximate algorithm $\alg$, mechanism $\mech_{crit}^{*}(\alg)$ has price of total anarchy at most $c + 1$.
%\end{thm}
%\begin{proof}
%Fix type profile $\types$, and let $D = \decls^1, \dotsc, \decls^T$ be a sequence of declarations in which all agents minimize external regret.  Suppose that $\mathbf{y}$ is an optimal allocation for $\types$.
%By Lemma \ref{lem.minregret}, $\frac{1}{T}\sum_t (\typei(\alg(\decls^t)) + \crit_i(y_i,\declsmi^t)) \geq \typei(y_i) - o(1)$.  Summing over all $i$, we have $\frac{1}{T}\sum_t\sum_i (\typei(\alg(\decls^t)) + \crit_i(y_i,\declsmi^t)) \geq SW_{OPT}(\types) - (n)(o(1))$.  By Lemma \ref{lem.loserindep}, this implies $\frac{1}{T}\sum_t\sum_i (\typei(\alg(\decls^t)) + c\decl_i^t(\alg(\decls^t))) \geq SW_{OPT}(\types) - (n)(o(1))$.  We know $\decl_i^t(\alg(\decls^t)) = \typei(\alg(\decls^t))$ for all $i$ and $t$ by Lemma \ref{lem.undom1}, so we conclude $(c+1)\frac{1}{T}\sum_t\sum_i \typei(\alg(\decls^t)) \geq SW_{OPT}(\types) - (n)(o(1))$.  Since the term hidden by the asymptotic notation vanishes with $T$ and does not depend on $n$, we obtain the desired result.
%\end{proof}
%
%%Theorem \ref{thm.regretmin} is very general, as it applies to a number of different problem settings in which loser-independent monotone approximation algorithms are known.  As a few particular examples, Theorem \ref{thm.regretmin} yields an $O(\sqrt{m})$ implementation of the combinatorial auction problem \cite{LOS-99}, an $s+1$ implementation of the combinatorial auction problem where sets are restricted to cardinality $s$ (using a simple greedy algorithm), an $O(m^{1/(B-1)})$ implementation of the unsplittable flow problem with minimum edge capacity $B$ \cite{BKV-05}, and an $O(R^{4/3})$ implementation of the combinatorial auction of convex bundles in the plane where $R$ is the maximum aspect ratio over all desired bundles \cite{BB-04}.
%
%The rate at which the welfare obtained by $\calm_{2}^{*}(\alg)$ converges to an average that is a $c+1$ approximation to optimal depends on the rate of convergence of players' external regret to $0$.  The average welfare obtained after $T$ rounds will have an additive loss of $(n)(r(T))$, where $r(T)$ is the average regret experienced by an agent after $T$ rounds.  Assuming that agents apply algorithms that minimize regret at a rate of $r(T) = o(1/\sqrt{T})$, which is attainable using the algorithm of Kalai and Vempala \cite{KV-05}, the additive error term is at most a constant when $T$ is at least quadratic in $n$.
%
%We note that, since agents experience no regret at a pure Nash equilibrium, an immediate corollary to Theorem \ref{thm.regretmin} is that mechanism $\mech_{crit}^{*}(\alg)$ has price of anarchy at most $c + 1$.  Indeed, Theorem \ref{thm.mixedNEepir} can be extended to show that mechanism $\mech_{crit}^{*}(\alg)$ has Bayesian price of anarchy at most $c+1$.  This result differs from Theorem \ref{thm.mixedNEepir} in that we do not require the additional assumption that agents do not overbid; only the weaker assumption that agents avoid dominated strategies.
%
%\subsection{Resilience to Irrational Strategies}
%
%Suppose that in addition to regret-minimizing agents, the auction participants include agents who do not follow rational strategies.  The only restriction we impose on the behaviour of such agents is that they do not overbid on any set; that is, $\decli(S) \leq \typei(S)$ for any $S$.  We can motivate this restriction either through our characterization of undominated strategies in Lemma \ref{lem.undom1}, or by thinking of irrational players as not understanding how to participate rationally in the auction, and hence likely to be conservative in the way that they bid.  Under this assumption, since Lemma \ref{lem.loserindep} holds for any declaration profile, we easily obtain the following generalization of Theorem \ref{thm.regretmin}.
%
%\begin{prop}
%\label{prop.resil}
%Let $\alg$ be a monotone greedy $c$-approximate algorithm.  Suppose agents have types $\types$, $D$ is a declaration sequence, and $N \subseteq [n]$ is a collection of agents that minimize regret in $D$ with respect to $\mech_{crit}^{*}(\alg)$.  Then if $\mathbf{y}$ is an optimal allocation for the agents in $N$, and the remaining agents never bid more than their true values on any set in $D$, then $\frac{1}{T}\sum_t SW(\allocs(\decls^t),\types) \geq \frac{1}{c+1}\sum_{i \in N}\typei(y_i) + |N|(o(1))$.
%\end{prop}
%\begin{proof}
%By Lemma \ref{lem.minregret} and summing over all $i \in N$, 
%\begin{align*}
%& \sum_{i \in N}\typei(y_i) - |N|(o(1)) \\ 
%\leq & \frac{1}{T}\sum_t\sum_{i\in N} (\typei(\alloci(\decls^t)) + \criti(y_i,\declsmi^t)) \\
%\leq & \frac{1}{T}\sum_t\sum_{i\in [n]} (\typei(\alloci(\decls^t)) + \criti(y_i,\declsmi^t)).
%\end{align*}  
%By Lemma \ref{lem.loserindep}, this implies $\frac{1}{T}\sum_t\sum_i (\typei(\alloci(\decls^t)) + c\decl_i^t(\alloci(\decls^t))) \geq \sum_{i \in N}\typei(y_i) - |N|(o(1))$.  The result then follows from the fact that $\decl_i^t(\alloci(\decls^t)) \leq \type_i^t(\alloci(\decls^t))$ for all $i$.
%\end{proof}
%
%\subsection{Importance of Strong Loser-Independence}
%
%We note that the strong loser-independence property is necessary for Theorem \ref{thm.regretmin}, as the following example demonstrates.
%
%\begin{example}
%Consider an auction problem in which no agent can be allocated more than $s$ objects, and moreoever $M = A \cup B$ where $|A| = |B| = m/2$ and the mechanism must either allocate objects in $A$ or objects in $B$, but not both.  Consider the algorithm that takes the maximum over two solutions: a greedy assignment of subsets of $A$, and a greedy assignment of subsets of $B$.  This algorithm is an $s+1$ approximation.
%
%Consider now an instance of the problem in which a single agent desires all of $B$ with value $1$, and each of $m/2$ agents desires a separate singleton in $A$ with value $1-\eps$.  Suppose that the agent desiring $B$ declares his valuation truthfully, but the other agents declare the zero valuation.  On this input, the algorithm obtains social welfare $1$, whereas $\frac{m}{2}(1-\epsilon)$ is possible.  However, this set of declarations forms a Nash equilibrium, and hence each agent has zero regret under this input profile.  Thus, even if agents minimize their regret, our mechanism may obtain a very poor approximation to the optimal social welfare over arbitrarily many auction rounds.  
%\end{example}



\section{Repeated Auctions and Regret Minimization}
\label{sec:regret}
%\allan{Slight change of section title and defintions for
%Repeated Auctions have been moved here. I have to check that 
%it reads smoothly now.}

Up to this point, we have considered the perfomance of mechanisms 
for one-shot allocation problems. We now turn to repeated auctions.  In this section, we focus on agents that apply regret minimizing strategies. 
%We recall the definitions of regret minimization and price of total anarchy as presented in Section~\ref{subsec:repeated}. We have the following theorem:
We consider an instance of a combinatorial allocation problem that proceeds in rounds.  The problem will be resolved by a direct revelation mechanism $\mech$, say with allocation algorithm $\alg$, which independently executes on each round of the auction.  As before, we will tend to write $\allocs$ for the allocation rule associated with algorithm $\alg$.  
%We will make use of the definitions of \emph{greedy} algorithms and \emph{strongly loser-independent} algorithms from 
%section \ref{sec:strong-loser-indep}.

We assume that neither the agent types nor the mechanism changes between rounds of the auction.  When the agents have types $\types$ and $D = (\decls^1, \decls^2, \dotsc, \decls^T, \ldots)$ is a sequence of declared valuation profiles, we
let $D_T$ denote  the length-$T$ prefix of $D$  and  we write $SW_{\alg}(D_T) = \frac{1}{T}\sum_t SW(\allocs(\decls^t),\types)$ for the average welfare obtained over the $T$ declarations in $D_T$.  We will sometimes replace subscript $\alg$ by $\mech$, in which case the social welfare is for the allocation rule of $\mech$.

Declaration sequence $D = (\decls^0, \decls^1, \dotsc)$ 
\emph{minimizes external regret} for agent $i$ if, for any fixed declaration $\decli$, the sequence of
finite prefixes satisfies $\sum_{t=1}^T \utili(\decl_i^t,\declsmi^t) \geq \sum_t \utili(\decli,\declsmi^t) + o(T)$.  That is, as $T$ increases, the per-round utility of agent $i$ approaches 
the utility of the optimal fixed strategy in hindsight. 
The {\it price of total anarchy} \cite{BHLR-08} is the worst-case ratio between optimal welfare and the welfare of a declaration that minimizes external regret; that is,
$$\sup_{\types,D} \frac{SW_{opt}(\types)}{SW(\calm(D),\types)}.$$

%We think of such (infinite) sequences as a {\em no-regret equilibrium} and
%consider sequences (and their average social welfare) generated by 
%mechanisms and in particular, mechanisms
%using greedy approximation allocation algorithms. The resulting price of
%anarchy concept for such a mechanism is then the {\em price of total anarchy} as introduced   
%in Blum et al \cite{BHLR-08}.; that is, the worst case ratio 
%over all such 
%regret minimization sequences. 
%As previously mentioned the 
%Roughgarden \cite{ROU-09} observes that 
%price of total anarchy is equivalent to the price of anarchy with
%respect to coarse correlated equlibirium.
% upper bounds the coarse correlated price of anarchy 
%and hence all the price of anarchy concepts in the one-shot setting.
%\allan{I am just saying in the above sentence that we have already indicated 
%that POA wrt coarse correlated equilibrium and POTA  and not restating 
%credit.}
%and if so where to do that. That is, the idea of randomizing
%over rounds. We said we might also mention how we can view price of total
%anarchy as a thought experiment in the one shot setting if that
%makes the relationship clearer. Looking at the current version of Roughgarden
%(for which I dont have a citation), he says that coarse correlated
%equilibirum is essentially equivalent to external no regret.} 
%The usefulness and performance  of mechanisms in this regret 
%minimization setting will  
% depend upon how the agents actually minimize their external regret and
%how fast the ``no-regret'' sequence converges.
%%, but how reasonable is it to assume that agents will do so?  i
%We recall that there is a simple and comutationally fast algorithm for minimizing regret due to Kalai and Vempala \cite{KV-05} for minimizing regret, known as ``follow the perturbed leader,'' which uses time polynomial in the number of actions that can be taken by the agent.  
%%They also provide an improved algorithm that minimizes regret for a linear optimization problem, which runs in time polynomial in the problem dimension \allan{Do we want to say what is the problem dinmension?}.  
%These algorithms require access to an exact best-response oracle, which chooses the strategy that maximizes utility given the expected outcomes of each strategy.  Kakade et al \cite{KKL-07} show how to use a $\gamma$-approximate best response oracle to achieve a $\gamma$-approximation to the best fixed declaration in hindsight.
%

\comment{
We now proceed with bounding the price of total anarchy obtained by $\mech_{2}^{*}(\alg)$.  Let $\mathbf{y}$ be an optimal assignment for types $\types$.  Suppose that $D = \decls^1, \dotsc, \decls^T$ is a no-regret sequence of declarations to our mechanism.  The definition of regret minimization then immediately implies the following. 

\begin{lem}
\label{lem.minregret}
If agent $i$ minimizes his external regret in bid sequence $D$, then 
\[\frac{1}{T}\sum_t (\typei(\alg(\decls^t)) + \criti^\alg(y_i,\declsmi^t)) \geq \typei(y_i) - o(1).\]
\end{lem}
\begin{proof}

Let $\decl'$ be the single-minded declaration for set $y_i$ at value $\typei(y_i)$.  From the definition of regret minimization,
\begin{align*}
\frac{1}{T}\sum_t & \utili(\decli^t,\declsmi^t) \geq \frac{1}{T}\sum_t \utili(\decl',\declsmi^t) - o(1) \\
& \geq \frac{1}{T}\sum_t \left(\typei(y_i) - \criti^\alg(y_i,\declsmi^t)\right) - o(1) \\
& = \typei(y_i) - \frac{1}{T}\sum_t \criti^\alg(y_i,\declsmi^t) - o(1).
\end{align*}
Since $\utili(\decli^t,\declsmi^t) \leq \typei(\alg(\decls^t))$ for all $t$, the result follows.
\end{proof}

Assume now that algorithm $\alg$ is strongly loser-independent.  We now recall from Lemma \ref{lem.greedy} that we can relate the value of the solution returned by an algorithm to the critical prices of the sets in an optimal solution.  Furthermore, we recall from Lemma \ref{lem.greedy1} that all greedy algorithms are strongly loser-independent.  We are now ready to proceed with bounding the price of total anarchy for mechanism $\mech_{2}^{*}(\alg)$.  
}

\begin{thm}
\label{thm.regretmin}
For any 
%monotone $c$-approximate algorithm 
$c$-approximate 
monotone strongly loser independent allocation rule
%$\msli$ 
$\alg$, mechanism $\mech_{1}(\alg)$ (respectively, $\mech_{2}^{*}(\alg)$) has price of total anarchy at most $\frac{c}{1-e^{-c}}$ (resp. $c + 1$).
\end{thm}
\begin{proof}
As observed by Blum and Mansour \cite{BlumM07} and Roughgarden \cite{ROU-09,Roughgarden12}, in the full information setting, price of total anarchy
is equal to price of anarchy with respect to 
coarse correlated equilibrium.
The result then follows immediately from Corollaries~\ref{cor:coarse} and \ref{cor:coarse.crit}.
%(more precisely, Corollary~\ref{cor:coarse}) and Theorem~\ref{thm.mixedNEcrit} as applied to
%coarse correlated equlibrium.
%
%
\comment{
Fix type profile $\types$, and let $D = \decls^1, \dotsc, \decls^T$ be a sequence of declarations in which all agents minimize external regret.  Suppose that $\mathbf{y}$ is an optimal allocation for $\types$.
By Lemma \ref{lem.minregret}, $\frac{1}{T}\sum_t (\typei(\alg(\decls^t)) + \crit_i(y_i,\declsmi^t)) \geq \typei(y_i) - o(1)$.  Summing over all $i$, we have $\frac{1}{T}\sum_t\sum_i (\typei(\alg(\decls^t)) + \crit_i(y_i,\declsmi^t)) \geq SW_{OPT}(\types) - (n)(o(1))$.  By Lemma \ref{lem.greedy}, 
%\ref{lem.loserindep}, 
this implies $\frac{1}{T}\sum_t\sum_i (\typei(\alg(\decls^t)) + c\decl_i^t(\alg(\decls^t))) \geq SW_{OPT}(\types) - (n)(o(1))$.  We know $\decl_i^t(\alg(\decls^t)) = \typei(\alg(\decls^t))$ for all $i$ and $t$ by Lemma \ref{lem.undom1}, so we conclude $(c+1)\frac{1}{T}\sum_t\sum_i \typei(\alg(\decls^t)) \geq SW_{OPT}(\types) - (n)(o(1))$.  Since the term hidden by the asymptotic notation vanishes with $T$ and does not depend on $n$, we obtain the desired result.
}
\end{proof}

One can suppose that each bidder employs an algorithm to determine which declaration to make at time $t$, given the bidding history up to time $t$.  We say that such an algoritm minimizes regret if employing the algorithm results in a sequence that minimizes external regret for the employing agent, for any bidding behavior of the other agents. 
Our interest in external regret minimization is motivated by the existence of simple and efficient bidding algorithms for minimizing regret.  Indeed, the price of total anarchy captures mechanism performance when agents apply reasonable learning techniques over the course of repeated participation.  In this sense we feel that this analysis is predictive of outcomes that would be observed in practice in a repeated auction.  The remainder of this section will be dedicated to elaborating on this point of computational tractability.

The standard algorithmic approach to minimizing external regret is the ``follow the perturbed leader'' (FPL) algorithm \cite{H-57,KV-05}, which requires time and space polynomial in the number of actions that can be taken by an agent.  Note that, in general, an action in a combinatorial auction mechanism corresponds to a declared valuation, of which there are super-polynomially many.  So FPL is not immediately applicable as an approach for arbitrary mechanisms.

We note, however, that the mechanism $\mech_2^*(\alg)$ (for a monotone strongly loser independent allocation rule 
%$\sli$ 
$\alg$) has some desirable properties that make it well-suited to the application of FPL techniques.  Recall that, for this mechanism, it suffices to consider only single-minded declarations from agents.  Furthermore, from Lemma \ref{lem.undom1}, all undominated strategies for agent $i$ involve selecting a single set $S_i$ and making a single-minded declaration for set $S_i$ at its true value $\typei(S_i)$.  An action in a given round therefore corresponds to a single set of items upon which to bid.

Of course, this still leaves an exponentially large (in $m$) space of actions, in general.  One should therefore consider the format in which agent valuations are represented.  For instance, a natural way to express an agent valuation is in XOR format~\cite{S-02,NIS-00}, which is a collection of single-minded valuations (i.e., set-value pairs) with the semantics that the value of a set $S$ will be the maximum specified value for any set contained in $S$.  The sets in the XOR representation are called the \emph{desired sets} of agent $i$.  This is an especially natural representation for many greedy algorithms, which typically iterate over the desired sets.

For a valuation represented in XOR format, it suffices to consider only bids for desired sets.  This is because any other bid, say for a set $S$, would be dominated by a bid for the desired set that determines the value of $S$.  Thus, if valuations are represented in XOR format, it suffices to consider a space of actions that is polynomial in the input size.  One can therefore apply FPL in an efficient manner, leading to the following conclusion.

%Our bounds on mechanism performance depend upon the agents actually minimizing their external regret, but how reasonable is it to assume that agents will do so?  We recall that there is a simple and efficient algorithm for minimizing regret due to Kalai and Vempala \cite{KV-05} for minimizing regret, known as ``follow the perturbed leader,'' which requires time polynomial in the number of actions that can be taken by the agent.  They also provide an improved algorithm that minimizes regret for a linear optimization problem, which runs in time polynomial in the problem dimension.  These algorithms require access to an exact best-response oracle, which chooses the strategy that maximizes utility given the expected outcomes of each strategy.  Kakade et al \cite{KKL-07} show how to use a $\gamma$-approximate best response oracle to achieve a $\gamma$-approximation to the best fixed declaration in hindsight.  

%The regret-minimization mechanism we construct in this paper will reduce the
%strategy space for a bidder to an optimization problem over the space of possible allocations to that bidder.  Using a follow-the-perturbed-leader approach, an agent can therefore minimize regret in time proportional to the number of desired sets in his valuation function.  If we assume the number of desired sets for each agent is polynomially small (e.g. in the model where agents provide these bids explicitly to the auction algorithm), then we conclude that agents can minimize regret efficiently.
%Alternatively, one could provide access to a best-response (or approximate best-response) oracle for the approximation algorithms being implemented, where the oracle must compute a best response to a distribution over possible declarations of the other agents.
%The ability to compute best-response choices is also a necessary component for the setting of best-response bidders, where the best-response assumption certainly requires that such strategies can be found efficiently.  
%
%In general, however, the space of possible allocations is exponentially large, and has exponential dimension as a linear problem.  Thus, any efficient best-response oracle (to a distribution over possible declarations of the other bidders) must depend on the model by which agents access their own preferences and the details of the problem setting and algorithm being implemented.  
%In general, we leave the construction of such oracles to the designers of mechanisms for specific problem domains. However, we observe that we can immediately apply the mecahnism $\mech_2^*$ such that it is possible to implement a best-repsonse oracle in polynomial time.

%\begin{thm}
%Computing a best response oracle for agent $i$ in mechanism $\mech_2^*(\alg)$ 
%can be done in time polynomial in $n$ and the number of sets desired by agent $i$. 
%\end{thm}

\begin{thm}
Computing a regret-minimizing for agent $i$ in mechanism $\mech_2^*(\alg)$ 
can be done in time, per round, that is polynomial in $n$ and the size of the XOR representation of agent $i$'s valuation. 
\end{thm}

%\begin{proof}
%Since the agent can effectively only make single-minded declarations, 
%his strategy space is equivalent to picking a desirable set and bidding 
%truthfully.
%\end{proof}




\section{Repeated Combinatorial Auctions and Best-Response Agents}
\label{sec:best-response}

%In general, however, the space of possible allocations is exponentially large, and has exponential dimension as a linear problem.  Thus, any efficient best-response oracle (to a distribution over possible declarations of the other bidders) must depend on the model by which agents access their own preferences and the details of the problem setting and algorithm being implemented.  We leave the construction of such oracles to the designers of mechanisms for specific problem domains.

%\allan{Cleaned up the first paragraph}
%\brendan{Consider moving the definitions related to best-response dynamics to this section.} \allan{I would prefer repeating the definition of best response
%dynamics rather than eliminating it in section 2.5. After reading the statement of Theorem 7.5, it is clear that we need to introduce or reintroduce some
%definitions here as the defs of SW in these repeated settings no 
%longer appears 
%in section 6. I don't think we need it now in section 6 but for sure we
%need to state explicitly the definitions in section 7. But I still do not
%think it hurts to leave section 2.5 as it is.}

In this section we consider the problem of designing mechanisms for agents that apply myopic best-response strategies asynchronously. 
%We shall also consider best response sequences of declarations. 
Declaration sequence $D = (\decls^0, \decls^1, \dotsc)$ is an instance of \emph{response dynamics} if for all prefixes, and for all $1 \leq t \leq T$, profiles $\decls^{t-1}$ and $\decls^t$ differ on the declaration of at most one player.  Response dynamics $D$ is an instance of \emph{best-response dynamics} if, whenever $\decls^{t-1}$ and $\decls^t$ differ on the declaration of agent $i$, $\decl_i^t$ maximizes agent $i$'s utility given the declarations of the other bidders. That is, $\decl_i^t \in \argmax_{\decl}\{\utili(\decl,\declsmi^t)\}$.
In our
model, 
agents are chosen for update uniformly at random to make a
best-response, one agent per round.
We will also 
assume that if a bidder is chosen for update but cannot improve his utility, he will choose to maintain his previous strategy.

%\allan{I removed the paragraph about the space of possible allocations being exponentially large and stuck it (commented out) at the start of section 8.}
%%In general, however, the space of possible allocations is exponentially large, and has exponential dimension as a linear problem.  Thus, any efficient best-response oracle (to a distribution over possible declarations of the other bidders) must depend on the model by which agents access their own preferences and the details of the problem setting and algorithm being implemented.  We leave the construction of such oracles to the designers of mechanisms for specific problem domains.

%\allan{ I removed the assumption about the initial empty bids and will change
%Lemma 7.3 accordingly. I think the assumption about not changing the bid if an agent cannot 
%improve the utility is fairly reasonable and for the time being I 
%am leaving it.} 
 
%We assume that    
%In order to keep our exposition clear, we will make two additional assumptions about the nature of the best-response behaviour (which can be removed, as we discuss in Sections \ref{sec:ex-post} and \ref{sec:best-response.general}).  First, we will suppose that in the initial state every bidder makes the empty declaration $\emptyset$.  Second, we suppose that if a bidder is chosen for update but cannot improve his utility, he will choose to maintain his previous strategy.  These assumptions will simplify the process of characterizing best-response strategies of agents, and in particular the statement of Lemma \ref{lem.separated} in the next section.  It is possible to remove these assumptions, at the cost of a minor modification to the mechanisms we propose.  We defer a more complete discussion to Section \ref{sec:best-response.general}. \allan{We might want to remove section 8.4 and just say that these
%areuppose that if a bidder is chosen for update but cannot improve his utility, he will choose to maintain his previous strategy. two reasonable assumptions and claim that they can be removed.}

We begin our analysis of myopic bidders by considering mechanism $\calm_{2}^{*}(\alg)$ from Section \ref{sec:ex-post} %and  \ref{sec:regret}, 
for a given monotone greedy algorithm $\alg$.  One might ask whether or not this mechanism converges to equilibrium under best-response dynamics.  A simple example shows that this is not the case: there are circumstances in which mechanism $\calm_{2}^{*}(\alg)$ has probability $0$ of ever converging to a pure Nash equilibrium via best-response dynamics, despite the existence of a pure equilibrium.
%\allan{A simple pure NE is 
%$\decl_1(\{d\}) = 6, \decl_2(\{b,c\}) = 5, \decl_3(\{c\} = \decl_4(\{d\}) = 0$. 
%But is this a convincing bidding strategy for players 3 and 4 even after 
%say players 1 and 2 have gone first? }  
%\brendan{Right, I would argue not; especially since players 3 and 4 each have a dominant strategy which is to bid truthfully (so it's not very convincing to have them bid 0).  So even though there do exist pure Nash equilibria for this instance, they aren't very compelling.} \allan{Should we indicate that the pure equilibria may not be very
%compelling? No one has even asked us about this so I guess it is
%understood that equilbria need not be compelling.}
%\brendan{Given the above discussion, it might make sense to say more about why best-response dynamics has reasonable predictive power.  That is, there do exist pure equilibria, but they aren't ``natural.''  So, if we don't believe players will actually randomize, the best response cycle is a reasonable outcome to expect in this example.  Do we believe this?  If so, it makes a compelling example.}
%\allan{I think I would just want to say that not all equilibria are compelling. 
%I do not follow your argument about the above response cycle being a reasonable 
%outcome.} 

%\allan{I distilled the bottom line of your argument about this example and
%added it as the last sentence in the example.} 
\begin{example}
Consider a combinatorial auction with 6 agents and 4 objects, say $\{a,b,c,d\}$, under the feasibility constraint that each agent can receive at most 2 items.  Let $\alg$ be the greedy allocation rule that allocates sets greedily by value.  We consider an input instance given by the following set of true values (where the value for a set not listed is taken to be the maximum over its subsets).

\begin{center}
\begin{tabular}{c|c|c}
player & set & value \\
\hline
$1$ & $\{a,b\}$ & $4$ \\
$1$ & $\{d\}$ & $6$ \\
$2$ & $\{a\}$ & $2$ \\
$2$ & $\{b,c\}$ & $5$ \\
$3$ & $\{c\}$ & $4$ \\
$4$ & $\{d\}$ & $5$ \\
\end{tabular}
\end{center}

Suppose the auction is resolved by mechanism $\calm_{2}^{*}(\alg)$, and agents apply best-response dynamics.  Agents $3$ and $4$ are single-minded and always maximize their utility by declaring truthfully.  Agents $1$ and $2$ each have a strategic choice to make when bidding: which of their two desired sets should they bid upon?  Note that once this decision is made, the way to bid is determined by Lemma \ref{lem.undom1} (i.e.~bid truthfully for the desired set).  It can be verified that from each of the resulting 4 possible declaration profiles, some player has incentive to change declaration.  Thus best-response dynamics need not converge to an equilibrium. 
%While the pure equilibrium in this example may not seem ``natural'', i
\end{example}

The non-convergence of best-response dynamics is not a technical artifact of the model.
Since the cyclic behavior described above employs undominated strategies by the players, we view it as a reasonable
outcome to expect in such an auction (especially if players are not willing or able to randomize).
%\allan{I think we are supposed to be using $\mech_2^*$, not $\mech_{2}^*$}
%\brendan{Say more about why it make sense to talk about the average, instead of (say) the minimum over the cycle.} 
%\allan{I assume you mean the maximum over the cycle. I don't have a compelling reason to say that the average makes more sense than the max. And one could consider other norms. I also don't think the average is less motivated.} 
The example above motivates a study of the total\footnote{While other measures are possible, such as the minimum welfare over the cycle, the total or average 
welfare seems to be more relevant to a mechanism and is consistent with the 
regret minimization measure in section \ref{sec:regret}.} (or equivalently 
the  
\emph{average}) social welfare of $\calm_{2}^{*}(\alg)$, over many rounds of best-response dynamics.  We conjecture that, on average, the best-response dynamics on mechanism $\calm_{2}^{*}(\alg)$ obtains an approximation to the optimal social welfare that is within a constant factor of the approximation ratio of the original algorithm $\alg$.  

\begin{conj}
\label{conj.best.response}
%If $\alg$ is a monotone greedy $c$-approximate algorithm, then $\calm_{2}^{*}(\alg)$ has $O(c)$ price of (myopic) sinking.
If $\alg$ is a $c$-approximate 
%\sli, 
monotone strongly loser independent allocation rule,
then $\calm_{2}^{*}(\alg)$ has $O(c)$ price of (myopic) sinking.
\end{conj}
%\allan{State as conjecture about stronlgly loser independent? Do we need
%to restate def of myopic sinking?}

%\brendan{todo -- think about this conjecture some more.  Do we still believe it's true?  Is there an easy counter-example?  Since we know more about PoA and smoothness now than we did 4 years ago, maybe it's more obvious...?} 
%\allan{I agree this is an important question. But I often say that the only bad conjecture is no conjecture , paraphrasing P.T. Barnum about publicity. We could soften this conjecture by saying ``$\calm_{2}^{*}(\alg)$ or some alternative transformation 
%from $\alg$ to a different mechanism $\calm_{2}^{**}(\alg)$''. I do not feel
%strongly about the conjecture but it seems plausisble.} 
We leave the resolution of Conjecture \ref{conj.best.response} as an open problem. More generally, although we believe mechanism $\calm_{2}^{*}(\alg)$ 
is an appropriate mechanism, the underlying goal is to have some black box transformation that converts a 
%monotone greedy $c$-approximation algorithm 
$c$-approximate $\sli$
into a mechanism with $O(c)$ price of myopic sinking. As partial progress, 
we will focus on two specific combinatorial auction settings:  the general combinatorial auction problem, and combinatorial auctions under a cardinality restriction.  For these two settings, we will construct alternative mechanisms and analyze the welfare they generate under best-response dynamics.

%we construct alternative mechanisms that are more amenable to best-response analysis.  These mechanisms are tailored specifically to the general combinatorial auction problem, and combinatorial auctions with cardinality-restricted sets.  


\subsection{The Approach}
\label{sec.approach}

Our bound on the price of total anarchy of $\mech_{2}^{*}(\alg)$ in Theorem \ref{thm.regretmin} and our price of anarchy bound in Theorem \ref{thm.mixedNEcrit} rely on a particular insight: if the social welfare of an auction outcome is low relative to the optimal welfare, then there must exist some agent $i$ for whom the optimal assignment has a low critical price.  We used this to argue that an outcome with low welfare cannot occur at equilibrium, since this agent $i$ could improve his utility by pursuing his allocation in the optimal assignment.

The difficulty when extending this intuition to asynchronous best-response dynamics is that even if an agent can improve his utility by attempting to win some set for which the critical price is low, it may be that he has no chance to do so because he is not chosen to update his bid.  Since each agent can expect to update his bid only once in every $n$ rounds, our concern is that an agent spends most rounds wishing to make a utility-improving bid, but that this improvement happens to be unavailable whenever it is that agent's turn to update.

We address this difficulty in two steps.  First, we modify our mechanism so that the social welfare is never much less than the sum of the bids of \emph{all} players - even those that are not allocated their desired sets.  We accomplish this by designing the mechanism so that a winning bid must be significantly larger than the sum of all conflicting bids.  This implies that if agent $i$ places a large bid on round $t$, then we can think of agent $i$ as making a large contribution to the social welfare even if she does not win her bid.  Second, we demonstrate that with high probability, in almost half of the rounds (or more), either agent $i$ places a large bid or else the critical price for her optimal allocation is high.  Thus, even though agent $i$ can modify her declaration only very infrequently, her (possibly indirect) contribution to the social welfare will still be large for approximately half of the rounds.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% CUT
%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%For the second step of the analysis,  our primary tool will be the following probabilistic lemma, which pertains to any mechanism in a best-response setting.  
%\brendan{The statement of this lemma is too confusing.  We should split it up: there should be an abstract lemma about Markov processes, then a more concrete lemma about best-response.  Instead of talking about ``properties,'' we should be more helpful to the reader and talk about what properties we mean.}
%Suppose $\calm$ is a mechanism, and $D$ is a sequence of best-response declarations for $\calm$.
%For any $\decls$, let $P_1(\declsmi)$ be some property of $\decls$ that does not depend on $\decli$, and let $P_2(\decli)$ be some property depending only on $\decli$.
%
%\begin{lem}
%\label{lem.numbad}
%Suppose that, for any $\decls$ such that $\decli$ is a best-response to $\declsmi$, $\lnot P_1(\declsmi)$ implies $P_2(\decli)$.  Then for all $\eps > 0$, if best-response dynamics is run for $T > \eps^{-1}n$ steps, there will be at least $(\frac{1}{2}-\eps)T$ steps $t$ for which either $P_1(\declsmi^t)$ or $P_2(\decl_i^t)$ is true, with probability at least $1 - e^{-T\eps^2/32n}$.
%\end{lem}
%\begin{proof}
%Note that $\decli$ is (on average) only a best response once in 
%every $n$ steps so that for most $t$, $\decli^t = \decli^{t-1}$.  Our proof will make use of the \emph{method of average bounded differences}.  We will begin by giving a brief statement of this technique; see, for example, \cite{DP-09} for a more thorough treatment.  Suppose that $z_1, \dotsc, z_n$ are (not necessarily independent) random variables, and let $f$ be real-valued function of $z_1, \dotsc, z_n$ satisfying the property that, for each $i \in [n]$ and any two values $a, a'$ that $z_i$ can assume, there is a non-negative value $c_i$ such that
%\[ | E[f|z_1, \dotsc, z_{i-1}; z_i = a] - E[f|z_1, \dotsc, z_{i-1}; z_i = a']| \leq c_i \]
%where the expectations are with respect to the values of $z_{i+1}, \dotsc, z_n$.  Then the method of average bounded differences states that $\Pr[f > \E[f] + \ell] \leq e^{-\ell^2/2c}$ for all $\ell > 0$, where $c = \sum_{i \in [n]}c_i^2$.
%
%We now proceed with the proof of the lemma.  We begin by defining a number of events, with respect to randomness in the instantiation of best-response dynamics.  For the remainder of the proof we will not distinguish between events and indicator variables for those events; that is, an event $Z$ will be associated with an indicator variable $Z$ such that $Z = 1$ if and only if the event occurs.  
%
%For each $t \in [T]$, let $B_i^t$ be the event that neither $P_1(\declsmi^t)$ nor $P_2(\decli^t)$ is true. 
%Let $A_i^t$ denote the event that $P_2(\decli^t)$ is true.
%Note that $A_i^t$ and $B_i^t$ are mutually exclusive.  Consider the steps in which either $A_i^t$ or $B_i^t$ occurs: let $R = \{ t \colon A_i^t \vee B_i^t \}$.  For all $r \leq |R|$, let $t(r)$ denote the $r$th largest element of $R$.  That is, $t(r)$ is the step at which either $A_i^t$ or $B_i^t$ is true for the $r$th time.  Let $C_r$ denote the event that $r \leq |R|$ and $B_i^{t(r)}$ is true.  That is, $C_r$ is the event that on the $r$th step in which either $A_i^t$ or $B_i^t$ occurs, it is $B_i^t$ that occurs.
%
%We then note that $T - \sum_{r \leq T} C_r$ is precisely the number of steps for which either $P_1(\declsmi^t)$ or $P_2(\decl_i^t)$ is true.  We therefore wish to show $Pr[\sum_{r \leq T} C_r > (\frac{1}{2}+\eps)T] < e^{-T\eps^2/32n}$, which implies our desired result.
%
%Pick $r$ and suppose that event $C_r$ occurs.  This implies that $B_i^{t(r)}$ occurs.  With probability $\frac{1}{n}$ agent $i$ is chosen for update on step $t(r)+1$.  Conditioning on that event, $A_i^{t(r)+1}$ must occur (by the assumption of the Lemma, using the fact 
%that $P_1(\declsmi)$ does not change on this step), and hence $t(r+1) = t(r) + 1$ and event $C_{r+1}$ does not occur.  We conclude $Pr[C_{r+1}|C_r] \leq (1-1/n)$. 
%%\allan{I added a clarifying remark that $P_1(\declsmi)$ did not change.}  \brendan{Ok.  Edited the new remark slightly.}
%   
%
%Next suppose that event $C_r$ does not occur; this implies that $A_i^{t(r)}$ occurs.
%With probability $(1-\frac{1}{n})$ agent $i$ is not chosen for update on step $t(r)+1$.  Conditioning on that event, $A_i^{t(r)+1}$ occurs (since $P_2$ depends only on the declaration of agent $i$, which does not change), and hence $t(r+1) = t(r)+1$ and $C_{r+1}$ does not occur.  We conclude $Pr[C_{r+1}|\neg C_r] \leq 1/n$.
%
%Let $D_1, D_2, \dotsc, D_T$ be a random walk on $\{0,1\}$ defined by $Pr[D_r|D_{r-1}] = (1-1/n)$, $Pr[D_r|\neg D_{r-1}] = 1/n$, and initial condition $D_0$.  Then our bounds above imply that $\sum_r C_r$ is stochastically dominated by $\sum_r D_r$, and hence 
%$Pr[\sum_r C_r > (\frac{1}{2}+\eps)T] \leq Pr[\sum_r D_r > (\frac{1}{2}+\eps)T]$.  It will therefore suffice to show that $Pr[\sum_{r \leq T} D_r > (\frac{1}{2}+\eps)T] < e^{-T\eps^2/32n}$.  
%
%The definition of $D_r$ yields 
%\begin{align*}
%Pr[D_r] & = \frac{1}{n}(1-Pr[D_{r-1}]) + \left(1-\frac{1}{n}\right)Pr[D_{r-1}] \\
%& = \frac{1}{n} + \left(1-\frac{2}{n}\right)Pr[D_r].  
%\end{align*}
%Solving this linear recurrence (with initial condition $D_0 \in \{0,1\}$) yields 
%\begin{align*}
%Pr[D_r] & = \frac{1}{2}(1-(1-2/n)^r) + D_0(1-2/n)^r \\
%& = \frac{1}{2} + (D_0 - \frac{1}{2})(1-2/n)^r.
%\end{align*}  
%Linearity of expectation then implies 
%\[ E\left[\sum_r D_r\right] = \frac{1}{2}T + \left(D_0 - \frac{1}{2}\right)\frac{n}{2}(1-(1-2/n)^{T+1}).\]
%From this we conclude that 
%\begin{equation}
%\label{eq.C.1}
%E\left[\sum_r D_r\right] < \frac{1}{2}T + \frac{n}{4}
%\end{equation} 
%and moreover 
%\begin{equation}
%\begin{split}
%\label{eq.C.2}
%\left|E\left[\left.\sum_r D_r \right| D_0=1\right] - E\left[\left.\sum_r D_r \right| D_0=0\right]\right| < \frac{n}{2}.
%\end{split}
%\end{equation}
%%
%Let $k = T/n$ and define random variables $F_1, \dotsc, F_k$ by $F_i = \sum_{r \in [in,(i+1)n-1]}D_r$.  Note that $F_i \in [0,n]$ for all $i$. Note also that
%\begin{equation}
%\label{eq.C.3}
%\sum_r D_r = \sum_i F_i.
%\end{equation}
%We would now like to apply the method of average bounded differences to random variables $F_1, \dotsc, F_k$ and function $f = \sum_i F_i$.  To do so, we must consider the expectation $\E[\sum_i F_i | F_1, \dotsc, F_{i-1}, F_i = \alpha]$ for $\alpha \in [0,n]$.  But note that the influence of $F_\ell$ on the values of $F_{\ell+1}, \dotsc, F_{k}$ is captured entirely by the value of $D_{(\ell+1)n-1}$, and from \eqref{eq.C.2} the influence of $D_{(\ell+1)n-1}$ on $\sum_{r = (\ell+1)n}^T D_r = \sum_{r=\ell+1}^k F_r$ is bounded by $\frac{n}{2}$.  Since the value of $F_\ell$ also influences the sum $\sum_i F_i$ directly by at most $n$ (due to its being included in the summation), we conclude that for all $\alpha,\alpha' \in [0,n]$,
%\begin{align*}
%& \left| \E\left[\left. \sum_j F_j \right| F_1, \dotsc, F_{i-1}, F_i = \alpha \right] - \E\left[\left. \sum_j F_j \right| F_1, \dotsc, F_{i-1}, F_i = \alpha' \right] \right| \leq 3n/2.
%\end{align*} 
%Thus, by the method of average bounded differences (and recalling that $k = T/n$), we conclude that 
%\begin{align}
%\label{eq.C.4}
%Pr\left[\sum_j F_j > \E\left[\sum_j F_j\right] + (\eps/2)T\right] \leq e^{-(T\eps/2)^2/2(3n/2)^2k} < e^{-T\eps^2/18n}.
%\end{align}
%Our final step is to bound $\E\left[\sum_j F_j\right] + (\eps/2)T$ from the left-hand side of \eqref{eq.C.4}.  Since $T > \eps^{-1}n$, we have from \eqref{eq.C.3} and \eqref{eq.C.1} that 
%\[\E\left[\sum_j F_j\right] + (\eps/2)T = \E\left[\sum_j D_j\right] + (\eps/2)T \leq \frac{1}{2}T + \frac{n}{4} + (\eps/2)T < \left(\frac{1}{2} + \eps\right)T.\]  
%Thus \eqref{eq.C.4} implies
%\[ Pr\left[\sum_j F_j > \left(\frac{1}{2} + \eps\right)T\right] < e^{-T\eps^2/32n}\] 
%and the result follows.
%\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% END CUT
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{A Mechanism for $s$-CAs}
\label{sec.mech.sCA}

Consider the $s$-CA problem, which is a combinatorial auction in which 
the feasibility constraint requires that no agent can be allocated more than $s$ objects.  
%\allan{Small quibble: in an CA we usually say that the valuation is monotone
%wrt set inclusion so for s-CAs we just say that the value of all sets are 
%determined by subsets of size at most s. Here we are imposing the small set 
%constraint by making it a feasibility constraint.} 
An algorithm that greedily assigns sets in descending order by value obtains an $s$-approximation.
%\footnote{For single-minded declarations as it is used in mechanism $\calm_{sCA%}$, the greedy algorithm is an $s$ approximation.}.  
%\allan{Since we only call $\alg_{sCA}$ after we simplify to single minded 
%bids, it seems that we have an $s$ approximation and we don't need 
%the footnote.} 
Call this algorithm $\alg_{sCA}$.  We will construct a mechanism $\calm_{sCA}$ based on $\alg_{sCA}$; it is described in Figure \ref{fig.mech.sCA}.  This algorithm simplifies incoming bids (in the same way as $\calm_{2}^{*}(\alg)$) and runs algorithm $\alg_{sCA}$ to find a potential allocation.  However, an additional condition for inclusion in the solution is imposed: the value declared for a set must be at least twice the sum of all bids for intersecting sets.  Potential allocations that satisfy this condition are allocated, and the mechanism charges critical prices (that is, the smallest value at which an agent would be allocated their set by $\calm_{sCA}$, which is not necessarily the same as the critical price for $\alg_{sCA}$).


\begin{figure}
\begin{center}
	\fbox{
		\begin{minipage}{0.9\linewidth}

\textbf{Mechanism} $\calm_{sCA}$:
\medskip
\hrule

\medskip

\textbf{Input:} Declaration profile $\decls = \decl_1, \dotsc, \decl_n$.

%\textbf{Output:} A partition $X_1, \dotsc, X_n$ of $M$.
%
\begin{tabbing}
%0. \= Remove all $\decli(S)$ for which $|S| > s$. \\
1. \= $\decl' \leftarrow $ \texttt{SIMPLIFY}$(\decls)$, \ \ \% say $\decli' = (S_i,v_i)$ \\
2. \> $(T_1, \dotsc, T_n) \leftarrow \alg_{sCA}(\decls')$.\\
3. \> For each $i$ such that $T_i \neq \emptyset$:\\
4. \> \quad \= $I \leftarrow \{j : S_j \cap T_i \neq \emptyset \}$. \ \ \% $I$ is the set of bids that intersect $S_i$ \\
5. \> \> $\tau_i \leftarrow 2\sum_{j \in I}\decl_j(S_j)$. \\
6. \> \> If $\decli'(T_i) \leq \tau_i$, set $T_i \leftarrow \emptyset$, $\tau_i \leftarrow 0$.\\
7. \> Allocate $T_1, \dotsc, T_n$ and charge $\tau_1, \dotsc, \tau_n$. \ \ \% Critical prices.
\end{tabbing}
		\end{minipage}
	}
			\caption[A best-response mechanism for the $s$-CA problem]{Mechanism $\calm_{sCA}$, an implementation of greedy algorithm $\alg_{sCA}$ for the $s$-CA problem.  This mechanism uses procedure \texttt{SIMPLIFY} from Figure \ref{fig.mech.regret} in Section \ref{sec.overbid}.}
			\label{fig.mech.sCA}
	\end{center}
\end{figure}

We note that since our mechanism implements a monotone algorithm and charges critical prices, Lemma \ref{lem.undom1} implies that undominated strategies for agent $i$ involve choosing a set $S_i$ and making a truthful 
single-minded bid for $S_i$ at value $\typei(S_i)$.  We will therefore assume that agents bid in this manner.
However, the  agent still has a strategic decision regarding which set $S_i$ to 
choose. 
%\allan{Added the last sentence here.}

We begin our analysis with some notation.  Suppose that $\decls$ is a declaration profile, where each $\decli$ is single-minded for some set $S_i$.  For any set $T$, define the set of bids \emph{intersecting} agent $i$'s bid for $T$ in $\decls$
%, $I_i(\decls,T)$, 
to be $I_i(\decls,T) = \{j : j \neq i, S_j \cap T \neq \emptyset\}$.  We also define $L_i(\decls,T) = \{j : j \in I_i(\decls,T), \decl_j(S_j) < \typei(T) \}$ to be the set of \emph{lower} intersecting bids.  We recursively define the set of \emph{ancestors}, 
$A_i(\decls,T)$, for agent $i$ with respect to $T$ and $\decls$;
%, $A_i(\decls,T)$, recursively; 
it is the set of all lower intersecting bids, plus all ancestors of those lower intersecting bids.  That is, 
\[  
  A_i(\decls,T) = L_i(\decls,T) \cup \bigcup_{j \in L_i(\decls,T)} A_j(\decls,S_j).
\]

We say that $\decls$ is \emph{separated for agent $i$} if $\decli(S_i) \geq 2\sum_{j \in L_i(\decls,S_i)}\decl_j(S_j)$.  Profile $\decls$ is \emph{separated} if it is separated for every bidder.  Since an agent gains positive utility in mechanism $\calm_{cSA}$ only if the declaration is separated for him, 
%and since the intial state is the empty declaration profile (which is separated), 
we draw the following conclusion.
\begin{lem}
\label{lem.separated}
If a declaration profile $\decls$ is separated, then it remains separated after a step of the best-response dynamics for mechanism $\calm_{sCA}$. 
%At each step of the best-response dynamics for mechanism $\calm_{sCA}$, the declaration profile submitted by the agents will be separated.
\end{lem}
\begin{proof}
%\allan{There is an abuse of notation here since we are using 
%$\decl'$ and $\decli'$ 
%for both the new declaration as wll as the delaration that is obtained after 
%simplifying. So lets say we change this to ${\tilde \decl}$. I would change  
%the rest of the proof to be consistent with this change. Alternatively we 
%can change the notation in the mechanism. I am not sure
%why the inclusion $L_j(\decls',S_j) \subseteq L_j(\decls,S_j)$ holds. It seems
%that all the allocated sets can change.} \brendan{I have made this change from $\decl'$ to $\tilde{\decl}$.  I also expanded the argument about the inclusion, to try to make it more clear.}
%We will show that if declaration profile $\decls$ is separated, then it remains separated after a step of the best-response dynamics.  The result then follows from our assumption that the initial state is the empty declaration (which is separated).
%
Suppose agent $i$ is chosen to update his bid, say from $\decli$ to $\tilde{\decli}$.  Let $\tilde{\decls} = (\tilde{\decli},\declsmi)$.  If agent $i$ cannot improve his utility then $\tilde{\decls} = \decls$, so $\tilde{\decls}$ is separated as required.  Suppose otherwise, so agent $i$ changes the set upon which he bids from, say, $S_i$ to $\tilde{S_i}$.  Since $\utili(\tilde{\decli},\declsmi) > 0$, it must be that $\tilde{\decli}(\tilde{S_i}) > 2\sum_{j \in I_i(\tilde{\decls},\tilde{S_i})} \decl_j(S_j)$.  This implies that $\tilde{\decls}$ is separated for agent $i$.  It remains to verify that $\tilde{\decls}$ is separated for each $j \neq i$.  Since $\tilde{\decls}$ is separated for agent $i$, it must be that $\tilde{\decli}(\tilde{S_i}) > \decl_j(S_j)$ for all $j$ such that $\tilde{S_i} \cap S_j \neq \emptyset$.  This then implies that $i \not\in L_j(\tilde{\decls},S_j)$ for each $j \neq i$.  Moreover, only the declaration of agent $i$ changes between $\decls$ and $\tilde{\decls}$, and hence $L_j(\tilde{\decls},S_j)$ and $L_j(\decls,S_j)$ can differ only on whether they include $i$.  We conclude that, for all $j \neq i$, either $L_j(\tilde{\decls},S_j) = L_j(\decls,S_j)$ or $L_j(\tilde{\decls},S_j) = L_j(\decls,S_j) \backslash \{i\}$.  In either case, $L_j(\tilde{\decls},S_j) \subseteq L_j(\decls,S_j)$, and hence $\sum_{k \in L_j(\tilde{\decls},S_j)} \tilde{\decl_k}(S_k) \leq \sum_{k \in L_j(\decls,S_j)} \decl_k(S_k)$. Therefore, since $\decls$ is separated for all $j \neq i$, $\tilde{\decls}$ must be separated for each $j \neq i$ as well.
\end{proof}

%for the remainder of this section 

Motivated by Lemma \ref{lem.separated}, we will focus on separated declaration profiles\footnote{More formally, we could
assume an initial empty declaration (which is trivially separated) 
so that by induction
all declarations will be separated. Alternatively, 
we can modify mechanism $\calm_{sCA}$ %and $\calm_{CA}$ 
so that, with vanishingly small probability, an alternative allocation rule is used.  This alternative rule chooses an agent at random, and assigns him all objects at no cost \emph{as long as the input declaration is separated for that agent}.  Thus, any separated declaration by agent $i$ results in positive expected utility.  Since any non-separated declaration by an agent results in a utility of $0$ for that agent, it must be that the utility-maximizing declaration by any agent must be separated.} for the remainder of this section. We will show that, for any separated declaration profile, $\calm_{sCA}$ extracts a constant fraction of the sum of all declared bids, as welfare.
%\allan{We say we will assume this but then keep repeating the assumption in 
%many propositions.} \brendan{I do think we should state this in proposition statements; so I changed the sentence above.}

\begin{lem}
\label{lem.separated.totalwelfare}
For all separated declarations $\decls$, $SW_{\mech_{sCA}}(\decls) \geq \frac{1}{2}\sum_i \decli(S_i)$.  
\end{lem}
\begin{proof}
%\allan{Might want to reverse the roles of $i$ and $j$ so that $i \notin N$
%and $j \in N$ to be consistent with Lemma 7.7. Also I think the current 
%$j \in A_i(\decls,S_j)$ should be $j \in A_i(\decls,S_i)$.} 
%\brendan{For $i$ and $j$, would it perhaps be better to switch the roles of $i$ and $j$ in Prop 7.7 instead?  What do you think?} 
%\allan{I agree, and I switched roles of i and j in proposition 7.7 as it is now more consistent with Proposition 7.5. I hope I made the switch without introducing any typos. Pleaase check to be sure. In that proof, the assertion that $k \in N$ is a little indirect due to the recursive nature of the ancestor function. Not sure if this needs to be explained?}
We first claim that, for each agent $i$,
\begin{equation}
\label{eq.sep1}
\decli(S_i) \geq \sum_{j \in A_i(\decls,S_i)} \decl_j(S_j).
\end{equation}
This follows by structural induction on the recursive definition of $A_i(\decls, T)$, since for each $i$ we have
\begin{align*}
\decli(S_i) & \geq 2\sum_{j \in L_i(\decls,S_i)} \decl_j(S_j) \\
& \geq \sum_{j \in L_i(\decls,S_i)} \decl_j(S_j) + \sum_{j \in L_i(\decls,S_i)} \sum_{k \in A_j(\decls,S_j)} \decl_k(S_k) \\
& \geq \sum_{j \in A_i(\decls,S_i)} \decl_j(S_j)
\end{align*}
where the first inequality follows by separatedness.

Let $N \subseteq [n]$ be the set of agents that receive non-empty sets in $\calm_{sCA}(\decls)$.  We next claim that for all $j \not\in N$, either $S_j = \emptyset$ or there exists some $i \in N$ such that $j \in A_i(\decls,S_i)$.  To see this, let $i$ be such that $\decli(S_i)$ is maximal, subject to $j \in A_i(\decls, S_i)$.  Note that such an $i$ must exist whenever $S_j \neq \emptyset$, though it could be that $i=j$. By maximality, the bid of $i$ cannot intersect with any larger bid in $\decls$, so $i$ is allocated a nonempty set by $\alg_{sCA}(\decls)$.  Moreover, by separatedness, the allocation to $i$ is not set to $\emptyset$ on line 6 of $\calm_{sCA}(\decls)$.  Thus $i \in N$, as claimed.  

Now, taking a sum over all $j \not\in N$ and applying \eqref{eq.sep1}, we can conclude
\begin{equation}
\label{eq.sep2}
\sum_{j \not\in N}\decl_j(S_j) \leq \sum_{i \in N}\sum_{j \in A_i(\decls,S_i)}\decl_j(S_j) \leq \sum_{i \in N}\decli(S_i).
\end{equation}
%By Lemma \ref{lem.separated.ancestors}, if set $S_i$ is allocated by $\mech_{sCA}$ then $\decli(S_i) \geq \sum_{j \in A_i(\decls,S_i)}\decl_j(S_j)$.  Let $N \subseteq [n]$ be the set of agents that receive non-empty sets in $\calm_{sCA}(\decls)$.  Proposition \ref{lem.separated.charge}
%implies that for all $j \not\in N$ there is some $i \in N$ such that $j \in A_i(\decls,S_i)$. 
We then have
\begin{align*}
\sum_i \decli(S_i) & = \sum_{i \in N}\decli(S_i) + \sum_{j \not\in N}\decl_j(S_j) \\
%& \leq SW_{\mech_{sCA}}(\decls) + \sum_{i \in N}\sum_{j \in A_i(\decls,S_i)}\decl_j(S_j) \\
& \leq \sum_{i \in N}\decli(S_i) + \sum_{i \in N}\decli(S_i) \\
& = 2SW_{\mech_{sCA}}(\decls)
\end{align*}
as required.
\end{proof}


%\begin{prop}
%\label{prop.sep.mech.sCA}
%If $\decls$ is separated, then $\mech_{sCA}$ allocates $S_i$ to agent $i$ precisely when $\decli(S_i) > \decl_j(S_j)$ for all $j \in I_i(\decls,S_i)$.
%\end{prop}
%\begin{proof}
%Note first that $\decli(S_i) > \decl_j(S_j)$ for all $S_j \cap S_i \neq \emptyset$ if and only if $\decli(S_i) > \max_{j \in I_i(S_i,\decls)}\decl_j(S_j)$.
%If this is true, then $S_i$ is allocated by $\alg_{sCA}(\decls)$.  Furthermore $L_i(S_i,\decls) = I_i(S_i,\decls)$, so (by separatedness) $\decli(S_i) > 2\sum_{j \in I_i(S_i,\decls)}\decl_j(S_j)$ and hence $S_i$ will be allocated by $\mech_{sCA}$.  On the other hand, if $\decli(S_i) \leq \max_{j \in I_i(S_i,\decls)}\decl_j(S_j)$, then certainly $\decli(S_i) \leq 2\sum_{j \in I_i(S_i,\decls)}\decl_j(S_j)$ so $S_i$ cannot be allocated by $\mech_{sCA}$.
%\end{proof}

%\begin{prop}
%\label{lem.separated.ancestors}
%If $\decls$ is separated then $\decli(S_i) \geq \sum_{j \in A_i(\decls,S_i)} \decl_j(S_j)$ for all $i$.
%\end{prop}
%\begin{proof}
%By induction on the definition of $A_i(\decls,T)$, we have that 
%\begin{align*}
%\decli(S_i) & \geq 2\sum_{j \in L_i(\decls,S_i)} \decl_j(S_j) \\
%& \geq \sum_{j \in L_i(\decls,S_i)} \decl_j(S_j) + \sum_{j \in L_i(\decls,S_i)} \sum_{k \in A_j(\decls,S_j)} \decl_k(S_k) \\
%& \geq \sum_{j \in A_i(\decls,S_i)} \decl_j(S_j).
%\end{align*}
%\end{proof}

%\allan{Fixed statement so that it only applies when everyone has had at least one best response.} \brendan{ok}

%\begin{prop}
%\label{lem.separated.charge}
%Assume that every agent has had at least one best reponse turn. 
%If $\decls$ is separated and mechanism $\calm_{sCA}$ allocates $\emptyset$ to agent $j$, then there exists $i$ such that $j \in A_i(\decls,S_i)$ and $\calm_{sCA}$ allocates $S_i$ to $i$.
%\end{prop}
%\begin{proof}
%Suppose $\mech_{sCA}$ allocates $\emptyset$ to agent $j$.  Let $N = \{ i : j \in A_i(\decls,S_i) \}$, and choose $i \in \argmax_{k \in N} \{ \decl_k(S_k) \}$. We claim that $\mech_{sCA}$ allocates $S_i$ to $i$.  If there exists $k$ such that $\decl_k(S_k) > \decl_i(S_i)$ and $S_k \cap S_i \neq \emptyset$, then $i \in L_k(\decls,S_k)$ and hence $k \in N$, contradicting the maximality of $i$.  Also, since $\decls$ is separated, there cannot exist $k$ such that $\decl_k(S_k) = \decl_i(S_i)$ and $S_k \cap S_i \neq \emptyset$.  Thus $\decl_k(S_k) < \decl_i(S_i)$ for all $k$ such that $S_k \cap S_i \neq \emptyset$, and hence $\mech_{sCA}$ allocates $S_i$ to agent $i$ by Proposition \ref{prop.sep.mech.sCA}.
%\end{proof}


%\begin{lem}
%\label{lem.separated.totalwelfare}
%For all separated declarations $\decls$, $SW_{\mech_{sCA}}(\decls) \geq \frac{1}{2}\sum_i \decli(S_i)$.  
%\end{lem}
%\begin{proof}
%%\allan{Might want to reverse the roles of $i$ and $j$ so that $i \notin N$
%%and $j \in N$ to be consistent with Lemma 7.7. Also I think the current 
%%$j \in A_i(\decls,S_j)$ should be $j \in A_i(\decls,S_i)$.} 
%\brendan{For $i$ and $j$, would it perhaps be better to switch the roles of $i$ and $j$ in Prop 7.7 instead?  What do you think?} 
%\allan{I agree, and I switched roles of i and j in proposition 7.7 as it is now more consistent with Proposition 7.5. I hope I made the switch without introducing any typos. Pleaase check to be sure. In that proof, the assertion that $k \in N$ is a little indirect due to the recursive nature of the ancestor function. Not sure if this needs to be explained?}
%By Lemma \ref{lem.separated.ancestors}, if set $S_i$ is allocated by $\mech_{sCA}$ then $\decli(S_i) \geq \sum_{j \in A_i(\decls,S_i)}\decl_j(S_j)$.  Let $N \subseteq [n]$ be the set of agents that receive non-empty sets in $\calm_{sCA}(\decls)$.  Proposition \ref{lem.separated.charge}
%implies that for all $j \not\in N$ there is some $i \in N$ such that $j \in A_i(\decls,S_i)$. Then
%\begin{align*}
%\sum_i \decli(S_i) & = \sum_{i \in N}\decli(S_i) + \sum_{i \not\in N}\decli(S_i) \\
%& \leq SW_{\mech_{sCA}}(\decls) + \sum_{i \in N}\sum_{j \in A_i(\decls,S_i)}\decl_j(S_j) \\
%& \leq SW_{\mech_{sCA}}(\decls) + \sum_{i \in N}\decli(S_i) \\
%& = 2SW_{\mech_{sCA}}(\decls)
%\end{align*}
%as required.
%\end{proof}

We are now ready to bound the price of sinking for $\mech_{sCA}$.  We will achieve the following bound.

\begin{thm}
\label{thm.best-response.1}
Choose $\eps > 0$ and suppose $D = d^1, \dotsc, d^T$ is an instance of best-response dynamics with random player order, where agents play undominated strategies, and $T > \eps^{-1}n$.  Then 
\[ SW_{\mech_{sCA}}(D) \geq \left(\frac{1-2\eps}{16s+8}\right)SW_{OPT}(\types) \]
with probability at least $1-ne^{-T\eps^2/32n}$.
\end{thm}

Before proving Theorem \ref{thm.best-response.1}, let us make some remarks.  If we take $\eps$ to be a small constant and assume $T = \Om(n^{1+\d})$ for some $\d > 0$, we conclude that $SW_{\mech_{sCA}}(D) > \frac{1}{O(s)}SW_{opt}(\types)$ with high probability.  Thus $\calm_{sCA}$ implements an $O(s)$ approximation to the $s$-CA problem for best-response bidders over sufficiently many rounds. In other words, $\calm_{sCA}$ has $O(s)$ price of (myopic) sinking.

We now begin with the proof of the theorem.  Let $\mathbf{y}$ be an optimal allocation with respect to the agents' true types $\types$.  
%We will apply Lemma \ref{lem.numbad} with $P_1(\declsmi)$ being the property that $\sum_{j \in I_i(\decls,y_i)}\decl_j(S_j) > \frac{1}{4}\vali(y_i)$, and with $P_2(\decli)$ being the property that $\decli(S_i) \geq \frac{1}{2}\vali(y_i)$.
%
For a given time step $t \leq T$, we will define a notion of ``good'' agents on step $t$.  Let $G_1^t$ denote the set of agents for which $\decli^t(S_i) \geq \frac{1}{2}\typei(y_i)$, and let $G_2$ denote the set of agents for which $\sum_{j \in I_i(\decls^t,y_i)}\decl_j^t(S_j) > \frac{1}{4}\typei(y_i)$.  That is, $G_1^t$ is the set of agents making relatively large bids at time $t$, and $G_2^t$ is the set of agents $i$ for whom a relatively large bid 
(that is, up to $\frac{1}{4} \typei(y_i)$) on set $y_i$ would not be a winning bid. 
%\allan{I added parenthetically that bid of $\frac{1}{4} \typei(y_i)$ would not be a winning bid.} %\allan{It seems that $G_2^t$ would be better described as the set of agents for whom a relatively large bid on set $y_i$ might not necessarily be a winning bid. So I am confused although the formal definition is how we are using $G_2^t$ in Lemma \ref{lem.goodevents.welfare}.} 
Write $G^t = G_1^t \cup G_2^t$; we will refer to $G^t$ as the set of good agents at time $t$.  

We will first argue that, at any given time $t$, the welfare achieved by our mechanism achieves a good approximation to the welfare of the optimal outcome, restricted to agents in $G^t$.  

\begin{lem}
\label{lem.goodevents.welfare}
For all $t$, $SW_{\mech_{sCA}}(\decls^t) \geq \frac{1}{8s+4}\sum_{i \in G^t}\typei(y_i)$.
\end{lem}
\begin{proof}
By Lemma \ref{lem.separated.totalwelfare} and the definition of $G_1^t$, we have
\begin{equation}
\label{eq.good1}
  SW_{\mech_{sCA}}(\decls^t) \geq \frac{1}{2}\sum_i \decli^t(S_i) \geq \frac{1}{2}\sum_{i \in G_1^t} \decli^t(S_i) \geq \frac{1}{4}\sum_{i \in G_1^t} \typei(y_i).
\end{equation}
Next, by Lemma \ref{lem.separated.totalwelfare} and the definition of $G_2^t$, we have
\begin{equation}
\label{eq.good2}
\begin{split}
SW_{\mech_{sCA}}(\decls^t) & \geq \frac{1}{2}\sum_i \decli^t(S_i) \\
& \geq \frac{1}{2}\cdot\frac{1}{s}\left(\sum_{i}\sum_{j \in I_i(\decls^t,y_i)}\decl_j^t(S_j) \right) \\
& \geq \frac{1}{2s} \sum_{i \in G_2^t}\sum_{j \in I_i(\decls^t,y_i)}\decl_j^t(S_j) \\
& \geq \frac{1}{8s} \sum_{i \in G_2^t}\type_i(y_i)
\end{split}
\end{equation}
where the second inequality follows because each set $S_j$ can intersect at most $|S_j| \leq s$ sets $y_i$, and the final inequality is by the definition of $G_2^t$.  Combining \eqref{eq.good1} and \eqref{eq.good2} yields the desired result. %\allan{Combining gives the bound $(\frac{1}{8s} + \frac{1}{4}) \sum_{i \in G^t} v_i(y_i)$ which is of course better than the stated bound.} 
\end{proof}
%\begin{equation}
%\label{eq.good}
%SW_{\mech_{sCA}}(\decls) \geq \frac{1}{8s+4}\sum_{i \in G^t} \typei(y_i)
%\end{equation}
%Also,
%$\sum_{i \in G_2}\sum_{j \in I_i(\decls,y_i)}\decl_j(S_j) \geq \frac{1}{4}\sum_{i \in G_2}\typei(y_i)$.  Since each $S_j$ can intersect at most $|S_j| \leq s$ sets $y_i$, we know that each $j$ appears in at most $s$ different sets of the form $I_i(\decls,y_i)$, and hence 
%\[\sum_{i \in G_2}\sum_{j \in I_i(\decls,y_i)}\decl_j(S_j) \leq s\sum_j \decl_j(S_j).\]  
%We conclude that $s\sum_j \decl_j(S_j) \geq \frac{1}{4}\sum_{i \in G_2}\typei(y_i)$.  Lemma \ref{lem.separated.totalwelfare} therefore implies that $(8s)SW_{\mech_{sCA}}(\decls) \geq \sum_{i \in G_2} \typei(y_i)$.

%We conclude that $(8s+4)SW_{\mech_{sCA}}(\decls) \geq \sum_{i \in G_1} \decli(S_i) + \sum_{i \in G_2} \decli(S_i)$, which implies the desired result.

In light of Lemma \ref{lem.goodevents.welfare}, our goal is to show that each agent is good sufficiently often over the course of an instance $D$ of best-response dynamics.  To this end, we will establish bounds on the probability that an agent lies in $G_1$ or $G_2$.

\begin{lem}
\label{lem.sep.response1}
For any $i$ and $t$, $\Pr[i \in G_1^{t+1} | i \in G_1^t] \geq 1 - \frac{1}{n}$.
\end{lem}
\begin{proof}
If $i \in G_1^t$, and $i$ is not selected by the best-response dynamics following round $t$, then it must be that $i \in G_1^{t+1}$.  Since $i$ is selected with probability $1/n$, the result follows.
\end{proof}

\begin{lem}
\label{lem.sep.response2}
For any $i$ and $t$, $\Pr[i \in G_1^{t+1} | i \not\in G^t] \geq \frac{1}{n}$.
\end{lem}
\begin{proof}
Suppose $i \not\in G^t$, and that $i$ is selected by the best-response dynamics process following round $t$.  Since $i \not\in G_2^t$, it must be that that $\crit_i(y_i,\declsmi) = 2\sum_{j \in I_i(\decls,y_i)}\decl_j(S_j)$ in mechanism $\mech_{sCA}$, so agent $i$ would obtain utility at least $\frac{1}{2}\typei(y_i)$ by making a single-minded declaration for set $y_i$ at value $\typei(y_i)$.  His utility-maximizing declaration must therefore make at least this much utility, and therefore is a bid for some set $S_i$ with $\typei(S_i) \geq \frac{1}{2}\typei(y_i)$.  Thus, with probability $\frac{1}{n}$, agent $i$ is selected and necessarily chooses $\decl_i^{t+1}$ such that $i \in G_1^{t+1}$.
\end{proof}

We now show that the above observations imply that any given agent will be in $G^t$ reasonably often, with high probability.  This will follow immediately from the following technical lemma, whose proof we defer:

\begin{lem}
\label{lem.numbad}
Suppose that $\{A^t\}_{t \leq T}$ and $\{B^t\}_{t \leq T}$ are sequences of binary random variables satisfying the following properties:
\begin{enumerate}
\item $A^t + B^t \leq 1$ for all $t$, 
\item $\Pr[A^{t+1}=1 | B^t=1 ] \geq \frac{1}{n}$ for all $t$, and 
\item $\Pr[A^{t+1}=1 | A^t=1 ] \geq 1 - \frac{1}{n}$ for all $t$.  
\end{enumerate}
Then $\Pr[ \sum_t B^t \geq (\frac{1}{2}+\epsilon)T ] \leq e^{-T\eps^2/32n}$.
\end{lem}

\begin{cor}
\label{cor.good.often}
For any agent $i$, with probability at least $1-e^{-T\eps^2/32n}$, agent $i$ will be in $G^t$ for at least $(\frac{1}{2}-\eps)T$ values of $t$.
\end{cor}
\begin{proof}
Let $A^t$ be the indicator for event $i \in G_1^t$, and let $B^t$ be the indicator for the event $i \not\in G^t$.  By Lemma \ref{lem.sep.response1} and Lemma \ref{lem.sep.response2}, we can apply Lemma \ref{lem.numbad} to conclude that $i \not\in G^t$ for at most $(\frac{1}{2}+\eps)T$ values of $t$, with the required probability. 
%\allan{Reading the lemmas literally, I think we have $B^t$ to be the indicator for the event that $i \not\in G_2^t$ and then conclude that 
%$i \not \in G_1^t$ for at most the $(\frac{1}{2}+\eps)T$ values of $t$, with the required probability.}  
\end{proof}


%\begin{prop}
%\label{prop.sep.response}
%If $\decls$ is separated and $\sum_{j \in I_i(\decls,y_i)}\decl_j(S_j) < \frac{1}{4}\typei(y_i)$, then any utility-maximizing declaration for agent $i$, $\decli'$, will be a single-minded declaration for some $S_i$ with $\decli'(S_i) \geq \frac{1}{2}\typei(y_i)$.
%\end{prop}
%\begin{proof}
%Note that $\crit_i(y_i,\declsmi) = 2\sum_{j \in I_i(\decls,y_i)}\decl_j(S_j)$ in mechanism $\mech_{sCA}$, so agent $i$ would obtain utility at least $\frac{1}{2}\typei(y_i)$ by making a single-minded declaration for set $y_i$ at value $\typei(y_i)$.  Thus his utility-maximizing declaration must make at least this much utility, and therefore is a bid for some set $S_i$ with $\typei(S_i) \geq \frac{1}{2}\typei(y_i)$.
%\end{proof}

We are now ready to prove the main result of this section.

\begin{proofof}{Theorem \ref{thm.best-response.1}}
%\allan{I changed $G_t$ to $G^t$.} \brendan{Ok.}
Corollary \ref{cor.good.often} implies that each agent $i$ will be in $G^t$ for at least $(\frac{1}{2}-\eps)T$ values of $t$, with probability at least $1-e^{-T\eps^2/32n}$.  The union bound then implies that this occurs for every agent with probability at least $1-ne^{-T\eps^2/32n}$.  Conditioning on the occurrance of this event, Lemma \ref{lem.goodevents.welfare} implies
\begin{align*}
SW_{\mech_{sCA}}(D) & = \frac{1}{T}\sum_t SW_{\mech_{sCA}}(\decls^t) \\
& \geq \frac{1}{(8s+4)T}\sum_t\sum_{i \in G^t} \typei(y_i) \\
& \geq \frac{1}{(8s+4)T}\sum_i T \left(\frac{1}{2}-\eps\right)\typei(y_i) \\
& \geq \left(\frac{1-2\eps}{16s+8}\right)SW_{OPT}(\types)
\end{align*}
which implies the required bound.  
\end{proofof}

\subsection{Proof of Lemma \ref{lem.numbad}}

Our proof will make use of the \emph{method of average bounded differences}.  We will begin by giving a brief statement of this technique; see, for example, \cite{DP-09} for a more thorough treatment.  Suppose that $z_1, \dotsc, z_n$ are (not necessarily independent) random variables, and let $f$ be real-valued function of $z_1, \dotsc, z_n$ satisfying the property that, for each $i \in [n]$ and any two values $a, a'$ that $z_i$ can assume, there is a non-negative value $c_i$ such that
\[ | E[f|z_1, \dotsc, z_{i-1}; z_i = a] - E[f|z_1, \dotsc, z_{i-1}; z_i = a']| \leq c_i \]
where the expectations are with respect to the values of $z_{i+1}, \dotsc, z_n$.  Then the method of average bounded differences states that $\Pr[f > \E[f] + \ell] \leq e^{-\ell^2/2c}$ for all $\ell > 0$, where $c = \sum_{i \in [n]}c_i^2$.

We now proceed with the proof of Lemma \ref{lem.numbad}.  First recall the statement of the lemma.
Suppose that $\{A^t\}_{t \leq T}$ and $\{B^t\}_{t \leq T}$ are sequences of binary random variables satisfying the following properties:
\begin{enumerate}
\item $A^t + B^t \leq 1$ for all $t$, 
\item $\Pr[A^{t+1}=1 | B^t=1 ] \geq \frac{1}{n}$ for all $t$, and 
\item $\Pr[A^{t+1}=1 | A^t=1 ] \geq 1 - \frac{1}{n}$ for all $t$.  
\end{enumerate}
We wish to prove that $\Pr[ \sum_t B^t \geq (\frac{1}{2}+\epsilon)T ] \leq e^{-T\eps^2/32n}$.

Consider the steps in which $A^t$ and $B^t$ are not both $0$; let $R = \{ t \colon A^t + B^t \geq 1 \}$ be this set of steps.  For all $r \leq |R|$, let $t(r)$ denote the $r$th largest element of $R$.  That is, $t(r)$ is the step at which either $A^t$ or $B^t$ is $1$ for the $r$th time.  Let $C^r$ denote the (indicator variable for the) event that on the $r$th step in which either $A^t$ or $B^t$ is $1$, it is $B^t$ that is $1$.  Then $\sum_{r \leq T} C_r = \sum_{t \leq T} B^t$, so it is enough to show that $Pr[\sum_{r \leq T} C^r > (\frac{1}{2}+\eps)T] < e^{-T\eps^2/32n}$.

Since $\Pr[ A^{t+1} = 1 | B^t = 1 ] \geq 1/n$, we have that $Pr[C_{r+1}|C_r] \leq (1-1/n)$.  Moreover, if $C_r$ does not occur, then $A^{t(r)}$ occurs, and hence (since $\Pr[ A^{t+1}=1 | A^t=1 ] \geq 1 - \frac{1}{n}$), $C_{r+1}$ occurs with probability at most $1/n$.  That is, $\Pr[C_{r+1}|\neg C_r] \leq 1/n$.

%Next suppose that event $C_r$ does not occur; this implies that $A_i^{t(r)}$ occurs.
%With probability $(1-\frac{1}{n})$ agent $i$ is not chosen for update on step $t(r)+1$.  Conditioning on that event, $A_i^{t(r)+1}$ occurs (since $P_2$ depends only on the declaration of agent $i$, which does not change), and hence $t(r+1) = t(r)+1$ and $C_{r+1}$ does not occur.  We conclude $Pr[C_{r+1}|\neg C_r] \leq 1/n$.
%
Let $D_1, D_2, \dotsc, D_T$ be a random walk on $\{0,1\}$ defined by $Pr[D_r|D_{r-1}] = (1-1/n)$, $Pr[D_r|\neg D_{r-1}] = 1/n$, and initial condition $D_0$.  Then our bounds above imply that $\sum_r C_r$ is stochastically dominated by $\sum_r D_r$, and hence 
$Pr[\sum_r C_r > (\frac{1}{2}+\eps)T] \leq Pr[\sum_r D_r > (\frac{1}{2}+\eps)T]$.  It will therefore suffice to show that $Pr[\sum_{r \leq T} D_r > (\frac{1}{2}+\eps)T] < e^{-T\eps^2/32n}$.  

The definition of $D_r$ yields 
\begin{align*}
Pr[D_r] & = \frac{1}{n}(1-Pr[D_{r-1}]) + \left(1-\frac{1}{n}\right)Pr[D_{r-1}] \\
& = \frac{1}{n} + \left(1-\frac{2}{n}\right)Pr[D_r].  
\end{align*}
Solving this linear recurrence (with initial condition $D_0 \in \{0,1\}$) yields 
\begin{align*}
Pr[D_r] & = \frac{1}{2}(1-(1-2/n)^r) + D_0(1-2/n)^r \\
& = \frac{1}{2} + (D_0 - \frac{1}{2})(1-2/n)^r.
\end{align*}  
Linearity of expectation then implies 
\[ E\left[\sum_r D_r\right] = \frac{1}{2}T + \left(D_0 - \frac{1}{2}\right)\frac{n}{2}(1-(1-2/n)^{T+1}).\]
From this we conclude that 
\begin{equation}
\label{eq.C.1}
E\left[\sum_r D_r\right] < \frac{1}{2}T + \frac{n}{4}
\end{equation} 
and moreover 
\begin{equation}
\begin{split}
\label{eq.C.2}
\left|E\left[\left.\sum_r D_r \right| D_0=1\right] - E\left[\left.\sum_r D_r \right| D_0=0\right]\right| < \frac{n}{2}.
\end{split}
\end{equation}
%
Let $k = T/n$ and define random variables $F_1, \dotsc, F_k$ by $F_i = \sum_{r \in [in,(i+1)n-1]}D_r$.  Note that $F_i \in [0,n]$ for all $i$. Note also that
\begin{equation}
\label{eq.C.3}
\sum_r D_r = \sum_i F_i.
\end{equation}
We would now like to apply the method of average bounded differences to random variables $F_1, \dotsc, F_k$ and function $f = \sum_i F_i$.  To do so, we must consider the expectation $\E[\sum_i F_i | F_1, \dotsc, F_{i-1}, F_i = \alpha]$ for $\alpha \in [0,n]$.  But note that the influence of $F_\ell$ on the values of $F_{\ell+1}, \dotsc, F_{k}$ is captured entirely by the value of $D_{(\ell+1)n-1}$, and from \eqref{eq.C.2} the influence of $D_{(\ell+1)n-1}$ on $\sum_{r = (\ell+1)n}^T D_r = \sum_{r=\ell+1}^k F_r$ is bounded by $\frac{n}{2}$.  Since the value of $F_\ell$ also influences the sum $\sum_i F_i$ directly by at most $n$ (due to its being included in the summation), we conclude that for all $\alpha,\alpha' \in [0,n]$,
\begin{align*}
& \left| \E\left[\left. \sum_j F_j \right| F_1, \dotsc, F_{i-1}, F_i = \alpha \right] - \E\left[\left. \sum_j F_j \right| F_1, \dotsc, F_{i-1}, F_i = \alpha' \right] \right| \leq 3n/2.
\end{align*} 
Thus, by the method of average bounded differences (and recalling that $k = T/n$), we conclude that 
\begin{align}
\label{eq.C.4}
Pr\left[\sum_j F_j > \E\left[\sum_j F_j\right] + (\eps/2)T\right] \leq e^{-(T\eps/2)^2/2(3n/2)^2k} < e^{-T\eps^2/18n}.
\end{align}
Our final step is to bound $\E\left[\sum_j F_j\right] + (\eps/2)T$ from the left-hand side of \eqref{eq.C.4}.  Since $T > \eps^{-1}n$, we have from \eqref{eq.C.3} and \eqref{eq.C.1} that 
\[\E\left[\sum_j F_j\right] + (\eps/2)T = \E\left[\sum_j D_j\right] + (\eps/2)T \leq \frac{1}{2}T + \frac{n}{4} + (\eps/2)T < \left(\frac{1}{2} + \eps\right)T.\]  
Thus \eqref{eq.C.4} implies
\[ Pr\left[\sum_j F_j > \left(\frac{1}{2} + \eps\right)T\right] < e^{-T\eps^2/32n}\] 
and the result follows.


%If we take $\eps$ to be a small constant and assume $T = \Om(n^{1+\d})$ for some $\d > 0$, we conclude that $SW_{\mech_{sCA}}(D) > \frac{1}{O(s)}SW_{opt}(\types)$ with high probability.  Thus $\calm_{sCA}$ implements an $O(s)$ approximation to the $s$-CA problem for best-response bidders over sufficiently many rounds. In other words, $\calm_{sCA}$ has $O(s)$ price of (myopic) sinking.


%\allan{There was a typo here; we had $\sum_{j \in I_i(\decls,y_i)}\decl_j(S_j) < \frac{1}{4}\vali(y_i)$ but it should be $>$ and not $<$.}  \brendan{Yes, I agree with that change.}  We now show that $P_1$ and $P_2$ satisfy the properties required by Lemma \ref{lem.numbad}.

%\begin{prop}
%\label{prop.sep.response}
%If $\decls$ is separated and $\sum_{j \in I_i(\decls,y_i)}\decl_j(S_j) < \frac{1}{4}\typei(y_i)$, then any utility-maximizing declaration for agent $i$, $\decli'$, will be a single-minded declaration for some $S_i$ with $\decli'(S_i) \geq \frac{1}{2}\typei(y_i)$.
%\end{prop}
%\begin{proof}
%Note that $\crit_i(y_i,\declsmi) = 2\sum_{j \in I_i(\decls,y_i)}\decl_j(S_j)$ in mechanism $\mech_{sCA}$, so agent $i$ would obtain utility at least $\frac{1}{2}\typei(y_i)$ by making a single-minded declaration for set $y_i$ at value $\typei(y_i)$.  Thus his utility-maximizing declaration must make at least this much utility, and therefore is a bid for some set $S_i$ with $\typei(S_i) \geq \frac{1}{2}\typei(y_i)$.
%\end{proof}

%For declaration profile $\decls$, let $G$ denote the set of agents $i$ for which either $\decli(S_i) > \frac{1}{4}\typei(y_i)$ or $\sum_{j \in I_i(\decls,y_i)}\decl_j(S_j) > \frac{1}{4}\typei(y_i)$.  We think of this as the set of agents with ``good'' bids.  %\allan{Another typo here as we had 
%%$\sum_{j \in I_i(\decls,y_i)}\decl_j(S_j) \geq \frac{1}{2}\typei(y_i)$ but
%%it should be $> \frac{1}{4}$ and not $\geq \frac{1}{2}$.} \brendan{I agree.} 
%We now bound the social welfare obtained by $\calm_{sCA}$ with respect to the optimal assignment to agents in $G$.

%\allan{Strictly speaking in the next Lemma we are getting the fraction $\frac{1}{4(2s+1)}$
%or equivalently $\frac{1}{8(s+\frac{1}{2})}$ and if we state it that way then 
%the theorem statement that follows also changes accordingly.} \brendan{Good point.  I fixed the statements.}
%\begin{lem}
%\label{lem.goodevents.welfare}
%$$SW_{\mech_{sCA}}(\decls) \geq \frac{1}{8s+4)}\sum_{i \in G}\typei(y_i).$$
%\end{lem}
%\begin{proof}
%Let $G_1$ denote the set of agents for which $\decli(S_i) \geq \frac{1}{2}\typei(y_i)$, and let $G_2$ denote the set of agents for which $\sum_{j \in I_i(\decls,y_i)}\decl_j(S_j) > \frac{1}{4}\typei(y_i)$, so that $G = G_1 \cup G_2$.
%
%By Lemma \ref{lem.separated.totalwelfare}, $SW_{\mech_{sCA}}(\decls) \geq \frac{1}{2}\sum_i \decli(S_i)$.  We then have
%\[ 
%  SW_{\mech_{sCA}}(\decls) \geq \frac{1}{2}\sum_i \decli(S_i) \geq \frac{1}{2}\sum_{i \in G_1} \decli(S_i) \geq \frac{1}{4}\sum_{i \in G_1} \typei(y_i).
%\]
%Also,
%$\sum_{i \in G_2}\sum_{j \in I_i(\decls,y_i)}\decl_j(S_j) \geq \frac{1}{4}\sum_{i \in G_2}\typei(y_i)$.  Since each $S_j$ can intersect at most $|S_j| \leq s$ sets $y_i$, we know that each $j$ appears in at most $s$ different sets of the form $I_i(\decls,y_i)$, and hence 
%\[\sum_{i \in G_2}\sum_{j \in I_i(\decls,y_i)}\decl_j(S_j) \leq s\sum_j \decl_j(S_j).\]  
%We conclude that $s\sum_j \decl_j(S_j) \geq \frac{1}{4}\sum_{i \in G_2}\typei(y_i)$.  Lemma \ref{lem.separated.totalwelfare} therefore implies that $(8s)SW_{\mech_{sCA}}(\decls) \geq \sum_{i \in G_2} \typei(y_i)$.
%
%We conclude that $(8s+4)SW_{\mech_{sCA}}(\decls) \geq \sum_{i \in G_1} \decli(S_i) + \sum_{i \in G_2} \decli(S_i)$, which implies the desired result.
%\end{proof}

%We are now ready to bound the average social welfare of our mechanism, over sufficiently many rounds, with respect to the approximation factor of algorithm $\alg$.


\subsection{A Mechanism for General CAs}
\label{sec.mech.CA}

%\allan{I have saved the previous version of this section in its entirety in
%a subsection of the appendix. Here I am just putting in a skeleton for 
%the new simplified randomized mechanism and refering to the appendix.} 

Consider the following algorithm for the general CA problem: first try greedily (by value) assigning sets of size at most $\sqrt{m}$,
then try allocating all items to the single agent with the highest declared value; return whichever of those two solutions generates more welfare.
%return either the resulting solution or the allocation that gives all items to a single agent, whichever generates more welfare.  
This algorithm is known to be an $O(\sqrt{m})$ approximation for the general CA problem \cite{Halldorsson00}. 
%\cite{MN-08}. 
%\allan{The $O(\sqrt{m})$ is more properly attributed to Halldorsson \cite{Halldorsson00} who gave the alg for set packing. I think the Mu'ahem and Nisan contribution might be to seeing that this can be made into a multi-minded CA but I am sure that
%Lehmann may have already said that. Lehmann gets credit for the greedy alg that
%sorts by $v_i(S)/|S|$ and Halldorsson states that as a personal communication.} 
We will construct a mechanism $\calm_{rCA}$ based on this algorithm; it is described in Figure \ref{fig.mech.rCA}.  The mechanism $\calm_{CA}$ essentially implements two copies of $\calm_{sCA}$ (as described in the previous section): one for sets of size at most $\sqrt{m}$ (which we will call $\calm_{\sqrt{m}CA}$), and one for allocating all objects to a single bidder. 
We call the latter the ``grand bundle mechanism'' $\calm_{GB}$, given in 
Figure~\ref{fig.mech.GB}.  
%\allan{Taking a look at what is being said next.} 
It is 
tempting to simply deterministically return whichever of the two solutions yields the largest social welfare. However, we will see in Appendix~\ref{sec.combine} that this deterministic 
algorithm will not always have a good POA in the one shot game. Instead we 
will consider a randomized mechanism in each round, one
that randomly chooses between $\calm_{\sqrt{m}CA}$  and $\calm_{GB}$. 
%\allan{We should now be able to utilize some of the material in the :?Instead
%next section.} 
%\allan{Commented out the pointing ahead to Appendix C which is
%being deleted (i.e. moved to a file).}
%In Appendix~\ref{sec.det-mech.CA}, we will construct a deterministic mechanism for the 
%general CA problem.   
\comment{We add one additional modification: with vanishingly small probability $\gamma$, $\calm_{CA}$ ignores bids for $M$ and behaves as $\calm_{\sqrt{m}CA}$.  The purpose of this modification is to encourage agents to bid on small sets, even when the presence of a high-valued bid for a large set would seem to indicate that bidding on small sets is fruitless.

\begin{figure}
\begin{center}
	\fbox{
		\begin{minipage}{0.9\linewidth}

\textbf{Mechanism} $\calm_{CA}$:

\hrule

\medskip

\textbf{Input:} Declaration profile $\decls = \decl_1, \dotsc, \decl_n$.

\begin{tabbing}
1.\ \ \ \= $\decl' \leftarrow $ \texttt{SIMPLIFY}$(\decls)$, say $\decli' = (S_i,v_i)$ \\
2. \> With probability $\gamma$:\\
3. \> \quad \= For all $i$ with $S_i = M$, $\decli' \leftarrow (\emptyset,0)$. \\
4. \> Let $(T_1, \dotsc, T_n) \leftarrow \mech_{\sqrt{m}CA}(\decls')$.\\
5. \> Let $T_i' \leftarrow \emptyset$ for all $i$.\\
6. \> If $\exists i : S_i = M$: \\
7. \> \> Let $j \leftarrow \argmax_j \{\decl_j'(M) : S_j = M\}$. \\
8. \> \> If $\decl_j'(S_j) > 2\sum_{k \neq j: S_k = M}\decl_k'(S_k)$: \\
9. \> \> \quad \= Set $T_j' \leftarrow M$. \\
10. \> If $\sum_i \decli(T_i) \geq \sum_i \decli(T_i')$, allocate $T_1, \dotsc, T_n$; otherwise allocate $T_1', \dotsc, T_n'$. \\
11. \> Charge critical prices.
\end{tabbing}

		\end{minipage}
	}
			\caption[A best-response mechanism for the general combinatorial allocation problem]{Mechanism $\calm_{CA}$, a best-response implementation of a greedy algorithm for the CA problem.  Parameter $\gamma > 0$ is an arbitrarily small positive constant.  Note $\calm_{\sqrt{m}CA}$ is $\calm_{sCA}$ from Figure \ref{fig.mech.sCA} with $s = \sqrt{m}$.}
			\label{fig.mech.CA}
	\end{center}
\end{figure}

}  %end comment

\begin{figure}
\begin{center}
        \fbox{
                \begin{minipage}{0.9\linewidth}

\textbf{Mechanism} $\calm_{GB}$:

\hrule

\medskip

\textbf{Input:} Declaration profile $\decls = \decl_1, \dotsc, \decl_n$.

\begin{tabbing}
\% A Vickery auction, thinking of 
$M$ as a single item. \\
%0. \= Remove all $\decli(S)$ for $S \neq M$ \ \ \% We can assume that
%every bidder has a bid for the grand bundle. \\  
%%1. \> $\decl' \leftarrow $ \texttt{SIMPLIFY}$(\decls)$  \  \ \% say $\decli' = (S_i,v_i)$ \\
%%1.\ \ \ \= $\decl' \leftarrow $ \texttt{SIMPLIFY}$(\decls)$  \  \ \% say $\decli' = (S_i,v_i)$ \\
%%2. \> With probability $\gamma$:\\
%%3. \> \quad \= For all $i$ with $S_i = M$, $\decli' \leftarrow (\emptyset,0)$. \\
%1. \> Let $(T_1, \dotsc, T_n) \leftarrow (\emptyset, \ldots, \emptyset)$ \\
%%5. \> Let $T_i' \leftarrow \emptyset$ for all $i$.\\
%%3. \> If $\exists i : S_i = M$: \\
%\allan{Changed the GB mechanism}  \\
%%\allan{Not sure if we need IF statement we can always just take $S_i$ to
%%be the $\max\{v_i(R), R \subseteq M\}$} \\
%%\brendan{Yes, I agree.  In fact, we should probably just simplify this mechanism completely,}\\
%%\brendan{and have it just accept a number from each agent, that being the agent's bid on}\\
%%\brendan{the grand bundle (which could be 0, if the bidder didn't bid on the grand bundle.)}\\
%2. \> \quad \=  Let $j \leftarrow \argmax_j \{\decl_j'(M) : S_j = M\}$. \\
%%%2. \> \quad \=  Let $j \leftarrow \argmax_j \{\decl_j(M)\}$. \\
%3. \> \> If $\decl_j'(S_j) > 2\sum_{k \neq j: S_k = M}\decl_k'(S_k)$: \\
%%%3. \> \> If $\decl_j(S_j) > 2\sum_{k \neq j: S_k = M}\decl_k(M)$: \\
%4. \> \> \quad \= Set $T_j \leftarrow M$. \\
%%10. \> If $\sum_i \decli(T_i) \geq \sum_i \decli(T_i')$, allocate $T_1, \dotsc, T_n$; otherwise allocate $T_1', \dotsc, T_n'$. \\
%5 \> Charge critical prices.
1. \ \ \= Let $(T_1, \dotsc, T_n) \leftarrow (\emptyset, \ldots, \emptyset)$. \\
%5. \> Let $T_i' \leftarrow \emptyset$ for all $i$.\\
%3. \> If $\exists i : S_i = M$: \\
%\allan{Changed the GB mechanism}  \\
%\allan{Not sure if we need IF statement we can always just take $S_i$ to
%be the $\max\{v_i(R), R \subseteq M\}$} \\
%\brendan{Yes, I agree.  In fact, we should probably just simplify this mechanism completely,}\\
%\brendan{and have it just accept a number from each agent, that being the agent's bid on}\\
%\brendan{the grand bundle (which could be 0, if the bidder didn't bid on the grand bundle.)}\\
2. \> Let $j \leftarrow \argmax_j \{\decl_j(M)\}$. \\
%%2. \> \quad \=  Let $j \leftarrow \argmax_j \{\decl_j(M)\}$. \\
%3. \> \> If $\decl_j'(S_j) > 2\sum_{k \neq j: S_k = M}\decl_k'(S_k)$: \\
%%3. \> \> If $\decl_j(S_j) > 2\sum_{k \neq j: S_k = M}\decl_k(M)$: \\
3. \> Set $T_j \leftarrow M$. \\
%10. \> If $\sum_i \decli(T_i) \geq \sum_i \decli(T_i')$, allocate $T_1, \dotsc, T_n$; otherwise allocate $T_1', \dotsc, T_n'$. \\
4. \> Return $(T_1, \dotsc, T_n)$ and charge critical prices.
\end{tabbing}

                \end{minipage}
        }
                        \caption[A best-response mechanism for the general combinatorial allocation problem]{Mechanism $\calm_{GB}$, an implementation of the grand bundle algorithm.}
                        \label{fig.mech.GB}
        \end{center}
\end{figure}

\begin{figure}
\begin{center}
        \fbox{
                \begin{minipage}{0.9\linewidth}

\textbf{Mechanism} $\calm_{rCA}$:

\hrule

\medskip

\textbf{Input:} Declaration profile $\decls = \decl_1, \dotsc, \decl_n$.
%\textbf{Input:} Declaration profile $\decls = \decl_1, \dotsc, \decl_n$.
%\allan{I took out the input declaration since it appears in the two mechanism.}

\begin{tabbing}
0 \ \ \= For each $i$, define $\decli'$ to be $\decli'(T) = \max_{S \subseteq T, |S| \leq \sqrt{m}}\{\decli(S)\}$. \\
1.\> With probability 1/2, return  $\calm_{sCA}(\decls')$ for $s = \sqrt{m}$. \\
%1.\ \ \= With probability 1/2, return  $\calm_{sCA}$ for $s = \sqrt{m}$ \\
2. \> Else return $\calm_{GB}(\decls)$.
\end{tabbing}

                \end{minipage}
        }
                        \caption[A best-response mechanism for the general combinatorial allocation problem]{Mechanism $\calm_{rCA}$, randomized mechanism for the CA problem.}
                        \label{fig.mech.rCA}
        \end{center}
\end{figure}

%\allan{The rest of this section has been replaced by the simplified proof as 
%discussed Wed, June 25.}
% for the
%randomized mechanism. But I am wondering about the fact that the grand bundle mechanism does not now force well separated bids. It seems that to simplify the proof of the Theorem for the overall mechanism we should just be able to refer to the small bundle proof where the only difference is that now the grand bundle takes care of all sets of size greater than $\sqrt{m}$}. 
%also going to kill (i.e. move to a file) appendix C. Do we want to have a statment that
%there s a deterministic mechanism? By the way, the mechanism in appendix C wasn't deterministic deterministic.}
The analysis of the average social welfare obtained by $\calm_{CA}$ closely follows the analysis for $\calm_{sCA}$.  Our high-level approach is to apply this analysis twice: once for allocations of sets of size at most $\sqrt{m}$, and once for allocations of all objects to a single bidder.  
%\allan{I think the next sentence should be removed.} The primary complicating factor is that the bidding choice of an agent may be influenced by the mechanism's choice of whether or not to allocate $M$ to a single bidder; this can be handled by a careful analysis of utility-maximizing declarations.  
The final result is the following.

\begin{thm}
\label{thm.best-response.2}
Choose $\eps > 0$ and suppose $D = d^1, \dotsc, d^T$ is an instance of best-response dynamics with random player order, where agents play undominated strategies, and $T > \eps^{-1}n$.  Then 
\[ SW_{\mech_{rCA}}(D) \geq \left(\frac{1-2\eps}{O(\sqrt{m})}\right)SW_{opt}(\types) \]
with probability at least $1-2ne^{-T\eps^2/32n}$.
\end{thm}

\begin{proof}
%\allan{Check the new wording of the proof.}
The initializations in mechanisms
$\calm_{GB}$, $\calm_{sCA}$, and $\calm_{rCA}$ ensure that declared valuations are used in the following way:
with probability $1/2$, only the bids on $M$ are used; otherwise, the mechanism considers only the single
highest bid on any set of size at most $\sqrt{m}$.  Given this, it is without loss of generality to assume that each declaration $\decli$ 
is the XOR of two single-minded bids: one for the set $M$ of all items, and one for a set $S_i$ of size at most $\sqrt{m}$.
%assigns
%value only to $M$ and to a single set $S_i$ of size at most $\sqrt{m}$.

Since $\calm_{GB}$ is a Vickrey auction on the grand bundle, undominated strategies for $\calm_{GB}$ involve bidding truthfully on $M$.
Also, our prior analysis of $\calm_{sCA}$ implies that undominated strategies for $\calm_{sCA}$ involve bidding truthfully on the chosen set $S_i$.
Thus, for mechanism $\calm_{rCA}$ the undominated strategies are precisely those that bid truthfully both on $M$ and on $S_i$. 

%(Note that
%such a bid is always possible, since $\vali(M) \geq \vali(S_i)$).
%
% we can assume that all declarations are for $M$ and 
%a single set of size at
%most $\sqrt{m}$. Furthermore, we know that bidding truthfully for these sets is
%a weakly dominant strategy.

%\allan{I would start the proof here. The following paragraph seems a little strange. The agent does not
%know which mechanism will be used so cannot declare a single minded 
%declaration.  I suggest we remove the first sentence and change the second 
%to the  following wording: ``Given the initialization in mechanism 
%$\calm_{GB}$, we can assume that all declarations are for $M$ or 
%a set of size at
%most $\sqrt{m}$. Furthermore, we know that bidding truthfully for these sets is
%a weakly dominant strategy.''}
%Note first that Lemma \ref{lem.undom1} applies to $\calm_{CA}$ for the same reason as $\calm_{sCA}$, so we will assume that all declarations in an instance of best-response dynamics are single-minded declarations, in which each $\decli$ is a bid for some set $S_i$ at value $\typei(S_i)$.  Also, we can assume that all single-minded declarations are for sets that are either $M$ or of size at most $\sqrt{m}$, since these are the only sets allocated by $\calm_{CA}$.

%\allan{Here will go a short one or two paragraph proof. The rest of this section will get removed (i.e. saved in a file). This is hand waving and may not 
%be correct technically but I want to make sure we have in mind the same idea.}

Let $\mathbf{y}$ be the optimal allocation in which each non-empty set has size greater than $\sqrt{m}$.  Then $SW(\mathbf{y},\types) \leq \sqrt{m}\max_i \typei(M)$, since there can be at most $\sqrt{m}$ non-empty sets in $\mathbf{y}$.   
%Using the same analysis as in Theorem \ref{thm.best-response.1}  and 
Since we can assume the agent will be bidding truthfully for set $M$ in 
$\calm_{GB}$ (and has no strategic decision as to which set to bid for as
in $\calm_{sCA}$), we can immediately apply the above $\sqrt{m}$ approximation analysis.  
Recalling that we are calling mechanism $\calm_{GB}$ with probability $\frac{1}{2}$ in
$\calm_{rCA}$, 
we conclude that 
%with probability at $1-2ne^{-T\eps^2/32n}$
\[ SW_{\mech_{rCA}}(D) \geq \frac{1}{2} \cdot \frac{1}{\sqrt{m}} SW(\mathbf{y},\types). \]
%\allan{I think the above happens with probability 1.}

Now let $\mathbf{z}$ be the optimal allocation of sets of size at most $\sqrt{m}$. From Theorem \ref{thm.best-response.1} and again recalling that we are 
calling $\calm_{\sqrt{m}CA}$ with probability $\frac{1}{2}$, we conclude that 
with probability at least $1-ne^{-T\eps^2/32n}$,
\[ SW_{\mech_{rCA}}(D) \geq \frac{1}{2} \cdot \frac{1-2\epsilon}{8\sqrt{m}}SW(\mathbf{z},\types). \]

Taking the union bound over the events described above, and noting that $SW_{OPT}(\types) \leq SW(\mathbf{z},\types) + SW(\mathbf{y},\types)$, we conclude that, with probability at least $1-ne^{-T\eps^2/32n}$,
\[ SW_{\mech_{rCA}}(D) \geq \frac{1-2\epsilon}{18 \sqrt{m}}SW_{OPT}(\types) \]
as required.




\end{proof}  

We conclude that mechanism $\calm_{rCA}$ implements an $O(\sqrt{m})$ approximation to the combinatorial auction problem for best-response bidders, with high probability, whenever $T = \Omega(n^{1+\delta})$ for $\delta > 0$.



